Maximizing Broadcast Throughput Under Ultra-Low-Power Constraints

Wireless object tracking applications are gaining popularity and will soon utilize emerging ultra-low-power device-to-device communication. However, severe energy constraints require much more careful accounting of energy usage than what prior art provides. In particular, the available energy, the differing power consumption levels for listening, receiving, and transmitting, as well as the limited control bandwidth must all be considered. Therefore, we formulate the problem of maximizing the throughput among a set of heterogeneous broadcasting nodes with differing power consumption levels, each subject to a strict ultra-low-power budget. We obtain the oracle throughput (i.e., maximum throughput achieved by an oracle) and use Lagrangian methods to design EconCast - a simple asynchronous distributed protocol in which nodes transition between sleep, listen, and transmit states, and dynamically change the transition rates. EconCast can operate in groupput or anyput modes to respectively maximize two alternative throughput measures. We show that EconCast approaches the oracle throughput. The performance is also evaluated numerically and via extensive simulations and it is shown that EconCast outperforms prior art by 6x - 17x under realistic assumptions. Moreover, we evaluate EconCast's latency performance and consider design tradeoffs when operating in groupput and anyput modes. Finally, we implement EconCast using the TI eZ430-RF2500-SEH energy harvesting nodes and experimentally show that in realistic environments it obtains 57% - 77% of the achievable throughput.

==> tex/algorithm.tex <==
\section{Proof Outline of Theorem~1}
\label{sec:algorithm}

\input{tex/proof_theorem}

In this section we provide an outline of the proof of Theorem~\ref{thm:convergence}. The complete proof can be found
% in Appendix~\ref{append:proof-convergence}.
in~\cite{econcast_techrep}.
The proof is based on a Markov Chain Monte Carlo (MCMC) approach~\cite{GBW13, ME08, JW10} from statistical physics. 

First, note that if the vector of multipliers $\mpliervec = [\mplier_i]$ freezes, {\name} generates the network state distribution described in the following lemma.
\begin{lemma}
\label{lem:dbe} % detailed balance equations
With fixed $\mpliervec$, the network Markov chain, resulted from overall interactions among the nodes according to the transition rates (\ref{eqn:rates2}), has the steady state distribution 
\begin{eqnarray}
\label{eqn:steady-state-prob}
\steadystate_{\statevec}^{\mpliervec} = \frac{1}{Z^{\mpliervec}} \exp \left[ \frac{1}{\oursigma} \left( \tput_{\statevec} - \sum\limits_{i:\state_i=l} \mpliernode{i} \listencost{i} - \sum\limits_{i:\state_i=x} \mpliernode{i} \xmitcost{i} \right) \right],
\end{eqnarray}
where $Z^{\mpliervec}$ is a normalizing constant so that $\sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec}^{\mpliervec} = 1$.
\end{lemma}
\begin{IEEEproof}
% The proof is followed by checking that the steady state distribution~\eqref{eqn:steady-state-prob} satisfies the detailed balance equations of the network Markov chain.
We assume $\oursigma = 1$ and drop the constant term $1/\oursigma$ for brevity. For network state $\statevec \in \statespace$, define $\setnodes_s(\statevec)$, $\setnodes_l(\statevec)$, and $\setnodes_x(\statevec)$ as the sets of nodes in sleep, listen, and transmit states, respectively, and their cardinalities as $\numnode_s(\statevec)$, $\numnode_l(\statevec)$, and $\numnode_x(\statevec)$, respectively. Note that $\numnode_s(\statevec) + \numnode_l(\statevec) + \numnode_x(\statevec) = \numnode$ and $\numnode_x(\statevec) \in \{0,1\}$. We also use $\statevec = (\setnodes_s(\statevec), \setnodes_l(\statevec), \setnodes_x(\statevec))$ to denote network state $\statevec$.

%We assume $\oursigma = 1$ and drop the constant term $1/\oursigma$ for brevity. For state $\statevec \in \statespace$, define $\setnodes_s(\statevec)$, $\setnodes_l(\statevec)$, and $\setnodes_x(\statevec)$ as the sets of nodes in sleep, listen, and transmit states, respectively, and their cardinalities as $\numnode_s(\statevec)$, $\numnode_l(\statevec)$, and $\numnode_x(\statevec)$, respectively. Note that $\numnode_s(\statevec) + \numnode_l(\statevec) + \numnode_x(\statevec) = \numnode$ and $\numnode_x(\statevec) \in \{0,1\}$. With a little abuse of notation, we also use $\statevec = (\setnodes_s(\statevec), \setnodes_l(\statevec), \setnodes_x(\statevec))$ to represent the network state $\statevec \in \statespace$.

For the capture version {\namecap}, we prove that the transition rates~\eqref{eqn:trans-rate-sl}, \eqref{eqn:trans-rate-ls}, \eqref{eqn:trans-rate-lx-cap}, and~\eqref{eqn:trans-rate-xl-cap} will drive the network Markov chain to a steady state with distribution~\eqref{eqn:steady-state-prob}, by checking that the {\em detailed balanced equations} hold. Let $r(\statevec, \statevec')$ denote the transition rate from state $\statevec$ to $\statevec'$. We consider the following cases.

% In {\namecap} (the capture version), the transition rates are given by~\eqref{eqn:trans-rate-sl}, \eqref{eqn:trans-rate-ls}, \eqref{eqn:trans-rate-lx-cap}, and~\eqref{eqn:trans-rate-xl-cap}. We prove that these transition rates will drive the network Markov chain to a steady state with distribution~\eqref{eqn:steady-state-prob}, by checking that the {\em detailed balanced equations} hold. Let $r(\statevec, \statevec')$ denote the transition rate from state $\statevec$ to $\statevec'$. We consider the following cases.

%% begin of proof
\noindent{\bf Case 1}: If node $i$ is in sleep state ($\state_i = s$), the only transition that can happen is to transition into listen state when the channel is clear, i.e., $\statevec = (\setnodes_s(\statevec), \setnodes_l(\statevec), \varnothing ) \to \statevec' = (\setnodes_s(\statevec) \setminus \{i\}, \setnodes_l(\statevec) \cup \{i\}, \varnothing )$.
In this case, $r(\statevec, \statevec') = \exp( -\mplier_i \listencost{i})$ and $r(\statevec', \statevec) = 1$.

\noindent{\bf Case 2}: If node $i$ is in listen state ($\state_{i} = l$), and transitions to sleep state, i.e., $\statevec = (\setnodes_s(\statevec), \setnodes_l(\statevec), \varnothing ) \to \statevec' = (\setnodes_s(\statevec) \cup \{i\}, \setnodes_l(\statevec) \setminus \{i\}, \varnothing )$.
In this case, $r(\statevec, \statevec') = 1$ and $r(\statevec', \statevec) = \exp( -\mplier_i \listencost{i})$.

\noindent{\bf Case 3}: If node $i$ is in listen state ($\state_{i} = l$) and transitions to transmit state, i.e., $\statevec = (\setnodes_s(\statevec), \setnodes_l(\statevec), \varnothing ) \to \statevec' = (\setnodes_s(\statevec), \setnodes_l(\statevec) \setminus \{i\}, \{i\} )$.
In this case, $r(\statevec, \statevec') = \exp( \mplier_i (\listencost{i} - \xmitcost{i}) )$ and $r(\statevec', \statevec) = \exp( -\numnode_l(\statevec'))$.

\noindent{\bf Case 4}: If node $i$ is in transmit state ($\state_{i} = x$), the only transition that can happen is to transition to listen state when its transmission is finished, i.e., $\statevec = (\setnodes_s(\statevec), \setnodes_l(\statevec), \{i\} ) \to \statevec' = (\setnodes_s(\statevec) \{i\}, \setnodes_l(\statevec) \cup \{i\}, \varnothing )$.
%%
In this case, $r(\statevec, \statevec') = \exp( -\numnode_l(\statevec))$ and $r(\statevec', \statevec) = \exp( \mplier_i(\listencost{i} - \xmitcost{i}) )$.

In all the cases, it can be verified that the detailed balance equations hold, i.e., $\steadystate_{\statevec} \cdot r(\statevec, \statevec') = \steadystate_{\statevec'} \cdot r(\statevec', \statevec)$.
For the non-capture version {\namenoncap}, similar detailed balance equations hold. Therefore, the steady state distribution~\eqref{eqn:steady-state-prob} satisfies the detailed balance equations of the network Markov chain which completes the proof.




\end{IEEEproof}

We then present an optimization problem {\namecp} as follows
%%
\begin{eqnarray}
\label{eqn:tput-lagrangian}
\hspace{-0.3in} {\namecp}
& \hspace{-0.1in} \max\limits_{\steadystatevec} & \sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec} \tput_{\statevec} - \oursigma \sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec} \log{\steadystate_{\statevec}}\\
& \hspace{-0.40in} \textrm{subject to} & (\ref{eqn:energy-constraint2}), ~(\ref{eqn:compute-frac2}), \textrm{and}~(\ref{eqn:pisum}) \nonumber,
\end{eqnarray}
%%
where $\oursigma$ is the positive constant used in {\name} (the counterpart in statistical physics is the temperature in systems of interacting particles).
Note that {\namecp} is a concave maximization problem and as $\oursigma \to 0$, the optimal value of {\namecp} approaches that of {\namelp}.
To solve {\namecp}, consider the Lagrangian function $\mathcal{L}(\steadystatevec,\mpliervec)$ formulated by moving the energy constraint (\ref{eqn:energy-constraint2}) into the objective (\ref{eqn:tput-lagrangian}) with a Lagrange multiplier $\mpliernode{i} \geq 0$ for each node $i$, i.e.,
%%
\begin{eqnarray}
\mathcal{L}(\steadystatevec, \mpliervec) = & \sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec} \tput_{\statevec} - \oursigma \sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec} \log{\steadystate_{\statevec}} \nonumber \\
& - \sum\nolimits_{i \in \setnodes} \left[ \mpliernode{i} (\listenfrac{i} \listencost{i} + \xmitfrac{i} \xmitcost{i} - \energybound{i}) \right].
\end{eqnarray}
%%
In view of (\ref{eqn:compute-frac2}) and (\ref{eqn:pisum}), given a vector of multipliers $\mpliervec$, it can be shown that the optimal $\steadystatevec^{\mpliervec} = [\steadystate_{\statevec}^{\mpliervec}]$ that maximizes $\mathcal{L}(\steadystatevec, \mpliervec)$ is exactly given by~(\ref{eqn:steady-state-prob}). Thus if {\name} knows the optimal choice of Lagrange multipliers, it can start with the optimal choice and the steady state distribution generated by {\name} will converge to the optimal solution to {\namecp}.

%% Centralized algorithm
\begin{algorithm}[!t]
\small
\caption{Gradient Descent Algorithm}
\label{alg:gradient-descent}
\begin{algorithmic}[1]
% input and init
\Statex\hspace{-\algorithmicindent}{\bf Input parameters}:
$\oursigma$, $\energyboundvec$, $\listencostvec$, and $\xmitcostvec$
\Statex\hspace{-\algorithmicindent}{\bf Initialization}:
$\listenfrac{i}(0)=\xmitfrac{i}(0)=\mpliernode{i}(0)=0, ~\forall i \in \setnodes$
% main loop
% \For{$k=1,2,\cdots$}
\State {\bf for} $k=1,2,\cdots$ {\bf do}
\State ~\quad $\stepsize{}(k) = 1/k$, compute $\steadystatevec(k)$ from (\ref{eqn:steady-state-prob}) using $\mpliervec = \mpliervec(k)$
% \For{$i=1,2,\cdots,\numnode$}
\State ~\quad {\bf for} $i=1,2,\cdots,\numnode$ {\bf do}
\State ~\quad~\quad Update $\mpliernode{i}(k)$, $\listenfrac{i}(k)$, and $\xmitfrac{i}(k)$ according to (\ref{eqn:update-lm}), (\ref{eqn:compute-frac})
% \EndFor
% \EndFor
\end{algorithmic}
\normalsize
\end{algorithm}
%%

Next, to find the optimal Lagrange multipliers $\mpliervec^*$, consider the dual $\mathcal{D}(\mpliervec) := \mathcal{L}(\steadystatevec^{\mpliervec}, \mpliervec)$ over $\mpliervec \succeq \bm{0}$ (here $\bm{0}$ is an $\numnode$-dimensional zero vector and $\succeq$ denotes component-wise inequality). Interestingly, it can be shown that the partial derivative of $\mathcal{D}(\mpliervec)$ with respect to $\mpliernode{i}$ is simply given by
\begin{equation}
\label{eq:gradient1}
\partial \mathcal{D} / \partial\mpliernode{i} = \energybound{i} - (\listenfrac{i} \listencost{i} + \xmitfrac{i} \xmitcost{i}),
\end{equation}
which is the difference between the power budget $\energybound{i}$ and the average power consumption of node $i$. Therefore, the dual can be minimized by using a gradient descent algorithm with inputs of step size $\stepsize_k > 0$, $\energyboundvec$, $\listencostvec$, and $\xmitcostvec$, which generates a state probability $\steadystatevec(k) ~(k = 1,2,\cdots)$. This algorithm is described in Algorithm~\ref{alg:gradient-descent} along with the following equations
%%
\begin{align}
\label{eqn:update-lm}
& \hspace{-0.1in} \mpliernode{i}(k) = \left[ \mpliernode{i}(k-1) - \stepsize_k (\energybound{i} - \listenfrac{i}(k) \listencost{i} - \xmitfrac{i}(k) \xmitcost{i}) \right]^+, \\
\label{eqn:compute-frac}
& \hspace{-0.1in} \listenfrac{i}(k) = \sum\nolimits_{\statevec \in \statespace_i^L} \steadystate_{\statevec}^{\mpliervec(k)}, ~\xmitfrac{i}(k) = \sum\nolimits_{\statevec \in \statespace_i^X} \steadystate_{\statevec}^{\mpliervec(k)}.
\end{align}
%%
Hence, with the right choice of step size $\stepsize_k$ (e.g., $\stepsize_k=1/k$), $\steadystatevec(k)$ converges to the optimal solution to {\namecp}.

%%
% how the gradient descent algorithm relates to the protocol
Finally, to arrive at a distributed solution, instead of computing the quantities $\listenfrac{i}$ and $\xmitfrac{i}$ directly according to (\ref{eqn:compute-frac}) (which is centralized with high complexity), we can approximate the difference between the power budget and the average power consumption~\eqref{eq:gradient1} by observing the dynamics of the energy storage level at each node.
Specifically, each node $i$ can update its Lagrange multiplier $\mpliernode{i}(k)$ based on the difference between its energy storage levels at the end and the start of an interval of length $\epoch_{k}$, divided by $\epoch_{k}$, as described by (\ref{eqn:update-lm-epoch}). Therefore $\mpliernode{i}$ is updated according to a ``noisy'' gradient descent. However, it follows from stochastic approximation (with Markov modulated noise) that by choosing step sizes and interval lengths as given in Theorem~\ref{thm:convergence}, these noisy updates will converge to $\mpliervec^*$ as $k \to \infty$ (see e.g., Theorem~1 of~\cite{jiang2009convergence}).
As mentioned in Section~\ref{ssec:distributed-param-choice}, the choice of parameters $\oursigma$, $\stepsize_{k}$, and $\epoch_{k}$ will affect the tradeoff between convergence time and the performance of {\name}. 


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../conext16"
%%% End:


==> tex/analysis_part1.tex <==

First, we present a concave optimization problem {\namecp}
%%
\begin{eqnarray}
\label{eqn:tput-lagrangian}
\hspace{-0.3in} {\namecp}
& \hspace{-0.1in} \max\limits_{\steadystatevec} & \sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec} \tput_{\statevec} - \oursigma \sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec} \log{\steadystate_{\statevec}}\\
& \hspace{-0.40in} \textrm{subject to} & (\ref{eqn:energy-constraint2}), ~(\ref{eqn:compute-frac2}), \textrm{and}~(\ref{eqn:pisum}) \nonumber,
\end{eqnarray}
%%
where $\oursigma$ is the positive constant used in {\name} (the counterpart in statistical physics is the temperature in systems of interacting particles).
Note that the optimal value of {\namecp} approaches that of {\namelp} as $\oursigma \to 0$.
To solve {\namecp}, consider the Lagrangian function $\mathcal{L}(\steadystatevec,\mpliervec)$ formulated by moving the energy constraint (\ref{eqn:energy-constraint2}) into the objective (\ref{eqn:tput-lagrangian}) with a Lagrange multiplier $\mpliernode{i} \geq 0$ for each node $i \in \setnodes$, i.e.,
%%
\begin{align*}
\mathcal{L}(\steadystatevec, \mpliervec) = & \sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec} \tput_{\statevec} - \oursigma \sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec} \log{\steadystate_{\statevec}} \\
& - \sum\nolimits_{i \in \setnodes} \left[ \mpliernode{i} (\listenfrac{i} \listencost{i} + \xmitfrac{i} \xmitcost{i} - \energybound{i}) \right].
\end{align*}
%%
In view of (\ref{eqn:compute-frac2}) and (\ref{eqn:pisum}), given a vector of multipliers $\mpliervec = [\mplier_{i}]$, the optimal $\steadystatevec^{\mpliervec} = [\steadystate_{\statevec}^{\mpliervec}]$ that maximizes $\mathcal{L}(\steadystatevec, \mpliervec)$ is exactly given by~(\ref{eqn:steady-state-prob}). Thus if {\name} knows the optimal choice of Lagrange multipliers, it can start with the optimal choice and the steady state distribution generated by {\name} will converge to the optimal solution to {\namecp}.

%% Centralized algorithm
\begin{algorithm}[!t]
\small
\caption{Gradient Descent Algorithm}
\label{alg:gradient-descent}
\begin{algorithmic}[1]
% input and init
\Statex\hspace{-\algorithmicindent}{\bf Input parameters}:
$\oursigma$, $\energyboundvec$, $\listencostvec$, and $\xmitcostvec$
\Statex\hspace{-\algorithmicindent}{\bf Initialization}:
$\listenfrac{i}(0)=\xmitfrac{i}(0)=\mpliernode{i}(0)=0, ~\forall i \in \setnodes$
% main loop
% \For{$k=1,2,\cdots$}
\State {\bf for} $k=1,2,\cdots$ {\bf do}
\State ~\quad $\stepsize{}(k) = 1/k$, compute $\steadystatevec(k)$ from (\ref{eqn:steady-state-prob}) using $\mpliervec = \mpliervec(k)$
% \For{$i=1,2,\cdots,\numnode$}
\State ~\quad {\bf for} $i=1,2,\cdots,\numnode$ {\bf do}
\State ~\quad~\quad Update $\mpliernode{i}(k)$, $\listenfrac{i}(k)$, and $\xmitfrac{i}(k)$ according to (\ref{eqn:update-lm}), (\ref{eqn:compute-frac})
% \EndFor
% \EndFor
\end{algorithmic}
\normalsize
\end{algorithm}
%%

Next, to find the optimal Lagrange multipliers $\mpliervec^*$, consider the dual $\mathcal{D}(\mpliervec) := \mathcal{L}(\steadystatevec^{\mpliervec}, \mpliervec)$ over $\mpliervec \succeq \bm{0}$ (here $\bm{0}$ is an $\numnode$-dimensional zero vector and $\succeq$ denotes component-wise inequality). Interestingly, it can be shown that the partial derivative of $\mathcal{D}(\mpliervec)$ with respect to $\mpliernode{i}$ is simply given by
\begin{equation}
\label{eq:gradient1}
\partial \mathcal{D} / \partial\mpliernode{i} = \energybound{i} - (\listenfrac{i} \listencost{i} + \xmitfrac{i} \xmitcost{i}),
\end{equation}
which is the difference between the power budget $\energybound{i}$ and the average power consumption of node $i$. Therefore, the dual can be minimized by using a gradient descent algorithm with inputs of step size $\stepsize_k > 0$, $\energyboundvec$, $\listencostvec$, and $\xmitcostvec$, which generates a state probability $\steadystatevec(k) ~(k = 1,2,\cdots)$. This algorithm is described in Algorithm~\ref{alg:gradient-descent} along with the following equations
%%
\begin{align}
\label{eqn:update-lm}
& \hspace{-0.1in} \mpliernode{i}(k) = \left[ \mpliernode{i}(k-1) - \stepsize_k (\energybound{i} - \listenfrac{i}(k) \listencost{i} - \xmitfrac{i}(k) \xmitcost{i}) \right]^+, \\
\label{eqn:compute-frac}
& \hspace{-0.1in} \listenfrac{i}(k) = \sum\nolimits_{\statevec \in \statespace_i^L} \steadystate_{\statevec}^{\mpliervec(k)}, ~\xmitfrac{i}(k) = \sum\nolimits_{\statevec \in \statespace_i^X} \steadystate_{\statevec}^{\mpliervec(k)}.
\end{align}
%%
Hence, with the right choice of step size $\stepsize_k$ (e.g., $\stepsize_k=1/k$), $\steadystatevec(k)$ converges to the optimal solution to {\namecp}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../conext16"
%%% End:


==> tex/analysis_v0.tex <==
\newpage
\section{Proof of Theorem 1}
\label{sec:analysis}

The proof of Theorem~\ref{thm:convergence} is based on a Markov Chain Monte Carlo (MCMC) approach~\cite{GBW13, ME08, JW10} from statistical physics and consists of three parts.
In the first part, we derive the steady state distribution of the network Markov chain under {\name} with given Lagrangian multiplier $\mpliervec = [\mplier_{i}]$.
In the second part, we present an alternative concave optimization problem whose optimal value approaches that of {\namelp} as $\oursigma \to 0$. We provide a centralized gradient descent algorithm based on Lagrangian method to solve this concave optimization problem.
In the third part, we show that nodes running {\name} update their Lagragian multipliers locally according to a ``noisy'' gradient descent and their Lagragian multipliers eventually converge to the optimal values with proper choices of step sizes and interval lengths as given in Theorem~\ref{thm:convergence}.

%% Begin of first part
% \subsection{The Perturbation Approach}
% \input{tex/analysis_part1}



%% End of first part




%%
\subsection{Steady State Distribution with Given $\oursigma$}
\label{ssec:proof-part-1}


First, note that if the vector of multipliers $\mpliervec = [\mplier_i]$ freezes, {\name} generates the network state distribution described in the following lemma.
\begin{lemma}
\label{lem:dbe} % detailed balance equations
With fixed $\mpliervec$, the network Markov chain, resulted from overall interactions among the nodes according to the transition rates (\ref{eqn:rates2}), has the steady state distribution 
\begin{eqnarray}
\label{eqn:steady-state-prob}
\steadystate_{\statevec}^{\mpliervec} = \frac{1}{Z^{\mpliervec}} \exp \left[ \frac{1}{\oursigma} \left( \tput_{\statevec} - \sum\limits_{i:\state_i=l} \mpliernode{i} \listencost{i} - \sum\limits_{i:\state_i=x} \mpliernode{i} \xmitcost{i} \right) \right],
\end{eqnarray}
where $Z^{\mpliervec}$ is a normalizing constant so that $\sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec}^{\mpliervec} = 1$.
\end{lemma}
\begin{IEEEproof}
% The proof is followed by checking that the steady state distribution~\eqref{eqn:steady-state-prob} satisfies the detailed balance equations of the network Markov chain.
We assume $\oursigma = 1$ and drop the constant term $1/\oursigma$ for brevity. For network state $\statevec \in \statespace$, define $\setnodes_s(\statevec)$, $\setnodes_l(\statevec)$, and $\setnodes_x(\statevec)$ as the sets of nodes in sleep, listen, and transmit states, respectively, and their cardinalities as $\numnode_s(\statevec)$, $\numnode_l(\statevec)$, and $\numnode_x(\statevec)$, respectively. Note that $\numnode_s(\statevec) + \numnode_l(\statevec) + \numnode_x(\statevec) = \numnode$ and $\numnode_x(\statevec) \in \{0,1\}$. We also use $\statevec = (\setnodes_s(\statevec), \setnodes_l(\statevec), \setnodes_x(\statevec))$ to denote network state $\statevec$.

%We assume $\oursigma = 1$ and drop the constant term $1/\oursigma$ for brevity. For state $\statevec \in \statespace$, define $\setnodes_s(\statevec)$, $\setnodes_l(\statevec)$, and $\setnodes_x(\statevec)$ as the sets of nodes in sleep, listen, and transmit states, respectively, and their cardinalities as $\numnode_s(\statevec)$, $\numnode_l(\statevec)$, and $\numnode_x(\statevec)$, respectively. Note that $\numnode_s(\statevec) + \numnode_l(\statevec) + \numnode_x(\statevec) = \numnode$ and $\numnode_x(\statevec) \in \{0,1\}$. With a little abuse of notation, we also use $\statevec = (\setnodes_s(\statevec), \setnodes_l(\statevec), \setnodes_x(\statevec))$ to represent the network state $\statevec \in \statespace$.

For the capture version {\namecap}, we prove that the transition rates~\eqref{eqn:trans-rate-sl}, \eqref{eqn:trans-rate-ls}, \eqref{eqn:trans-rate-lx-cap}, and~\eqref{eqn:trans-rate-xl-cap} will drive the network Markov chain to a steady state with distribution~\eqref{eqn:steady-state-prob}, by checking that the {\em detailed balanced equations} hold. Let $r(\statevec, \statevec')$ denote the transition rate from state $\statevec$ to $\statevec'$. We consider the following cases.

% In {\namecap} (the capture version), the transition rates are given by~\eqref{eqn:trans-rate-sl}, \eqref{eqn:trans-rate-ls}, \eqref{eqn:trans-rate-lx-cap}, and~\eqref{eqn:trans-rate-xl-cap}. We prove that these transition rates will drive the network Markov chain to a steady state with distribution~\eqref{eqn:steady-state-prob}, by checking that the {\em detailed balanced equations} hold. Let $r(\statevec, \statevec')$ denote the transition rate from state $\statevec$ to $\statevec'$. We consider the following cases.

%% begin of proof
\noindent{\bf Case 1}: If node $i$ is in sleep state ($\state_i = s$), the only transition that can happen is to transition into listen state when the channel is clear, i.e., $\statevec = (\setnodes_s(\statevec), \setnodes_l(\statevec), \varnothing ) \to \statevec' = (\setnodes_s(\statevec) \setminus \{i\}, \setnodes_l(\statevec) \cup \{i\}, \varnothing )$.
In this case, $r(\statevec, \statevec') = \exp( -\mplier_i \listencost{i})$ and $r(\statevec', \statevec) = 1$.

\noindent{\bf Case 2}: If node $i$ is in listen state ($\state_{i} = l$), and transitions to sleep state, i.e., $\statevec = (\setnodes_s(\statevec), \setnodes_l(\statevec), \varnothing ) \to \statevec' = (\setnodes_s(\statevec) \cup \{i\}, \setnodes_l(\statevec) \setminus \{i\}, \varnothing )$.
In this case, $r(\statevec, \statevec') = 1$ and $r(\statevec', \statevec) = \exp( -\mplier_i \listencost{i})$.

\noindent{\bf Case 3}: If node $i$ is in listen state ($\state_{i} = l$) and transitions to transmit state, i.e., $\statevec = (\setnodes_s(\statevec), \setnodes_l(\statevec), \varnothing ) \to \statevec' = (\setnodes_s(\statevec), \setnodes_l(\statevec) \setminus \{i\}, \{i\} )$.
In this case, $r(\statevec, \statevec') = \exp( \mplier_i (\listencost{i} - \xmitcost{i}) )$ and $r(\statevec', \statevec) = \exp( -\numnode_l(\statevec'))$.

\noindent{\bf Case 4}: If node $i$ is in transmit state ($\state_{i} = x$), the only transition that can happen is to transition to listen state when its transmission is finished, i.e., $\statevec = (\setnodes_s(\statevec), \setnodes_l(\statevec), \{i\} ) \to \statevec' = (\setnodes_s(\statevec) \{i\}, \setnodes_l(\statevec) \cup \{i\}, \varnothing )$.
%%
In this case, $r(\statevec, \statevec') = \exp( -\numnode_l(\statevec))$ and $r(\statevec', \statevec) = \exp( \mplier_i(\listencost{i} - \xmitcost{i}) )$.

The detailed balance equations hold in all the above cases, i.e., $\steadystate_{\statevec} \cdot r(\statevec, \statevec') = \steadystate_{\statevec'} \cdot r(\statevec', \statevec)$.
For the non-capture version {\namenoncap}, similar detailed balance equations hold.
% Therefore, the steady state distribution~\eqref{eqn:steady-state-prob} satisfies the detailed balance equations of the network Markov chain which completes the proof.



\end{IEEEproof}


%%
\subsection{The Perturbation Approach}

We then present an optimization problem {\namecp} as follows
%%
\begin{eqnarray}
\label{eqn:tput-lagrangian}
\hspace{-0.3in} {\namecp}
& \hspace{-0.1in} \max\limits_{\steadystatevec} & \sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec} \tput_{\statevec} - \oursigma \sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec} \log{\steadystate_{\statevec}}\\
& \hspace{-0.40in} \textrm{subject to} & (\ref{eqn:energy-constraint2}), ~(\ref{eqn:compute-frac2}), \textrm{and}~(\ref{eqn:pisum}) \nonumber,
\end{eqnarray}
%%
where $\oursigma$ is the positive constant used in {\name} (the counterpart in statistical physics is the temperature in systems of interacting particles).
Note that {\namecp} is a concave maximization problem and as $\oursigma \to 0$, the optimal value of {\namecp} approaches that of {\namelp}.
To solve {\namecp}, consider the Lagrangian function $\mathcal{L}(\steadystatevec,\mpliervec)$ formulated by moving the energy constraint (\ref{eqn:energy-constraint2}) into the objective (\ref{eqn:tput-lagrangian}) with a Lagrange multiplier $\mpliernode{i} \geq 0$ for each node $i$, i.e.,
%%
\begin{eqnarray}
\mathcal{L}(\steadystatevec, \mpliervec) = & \sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec} \tput_{\statevec} - \oursigma \sum\nolimits_{\statevec \in \statespace} \steadystate_{\statevec} \log{\steadystate_{\statevec}} \nonumber \\
& - \sum\nolimits_{i \in \setnodes} \left[ \mpliernode{i} (\listenfrac{i} \listencost{i} + \xmitfrac{i} \xmitcost{i} - \energybound{i}) \right].
\end{eqnarray}
%%
In view of (\ref{eqn:compute-frac2}) and (\ref{eqn:pisum}), given a vector of multipliers $\mpliervec$, it can be shown that the optimal $\steadystatevec^{\mpliervec} = [\steadystate_{\statevec}^{\mpliervec}]$ that maximizes $\mathcal{L}(\steadystatevec, \mpliervec)$ is exactly given by~(\ref{eqn:steady-state-prob}). Thus if {\name} knows the optimal choice of Lagrange multipliers, it can start with the optimal choice and the steady state distribution generated by {\name} will converge to the optimal solution to {\namecp}.

%% Centralized algorithm
\begin{algorithm}[!t]
\small
\caption{Gradient Descent Algorithm}
\label{alg:gradient-descent}
\begin{algorithmic}[1]
% input and init
\Statex\hspace{-\algorithmicindent}{\bf Input parameters}:
$\oursigma$, $\energyboundvec$, $\listencostvec$, and $\xmitcostvec$
\Statex\hspace{-\algorithmicindent}{\bf Initialization}:
$\listenfrac{i}(0)=\xmitfrac{i}(0)=\mpliernode{i}(0)=0, ~\forall i \in \setnodes$
% main loop
% \For{$k=1,2,\cdots$}
\State {\bf for} $k=1,2,\cdots$ {\bf do}
\State ~\quad $\stepsize{}(k) = 1/k$, compute $\steadystatevec(k)$ from (\ref{eqn:steady-state-prob}) using $\mpliervec = \mpliervec(k)$
% \For{$i=1,2,\cdots,\numnode$}
\State ~\quad {\bf for} $i=1,2,\cdots,\numnode$ {\bf do}
\State ~\quad~\quad Update $\mpliernode{i}(k)$, $\listenfrac{i}(k)$, and $\xmitfrac{i}(k)$ according to (\ref{eqn:update-lm}), (\ref{eqn:compute-frac})
% \EndFor
% \EndFor
\end{algorithmic}
\normalsize
\end{algorithm}
%%

Next, to find the optimal Lagrange multipliers $\mpliervec^*$, consider the dual $\mathcal{D}(\mpliervec) := \mathcal{L}(\steadystatevec^{\mpliervec}, \mpliervec)$ over $\mpliervec \succeq \bm{0}$ (here $\bm{0}$ is an $\numnode$-dimensional zero vector and $\succeq$ denotes component-wise inequality). Interestingly, it can be shown that the partial derivative of $\mathcal{D}(\mpliervec)$ with respect to $\mpliernode{i}$ is simply given by
\begin{equation}
\label{eq:gradient1}
\partial \mathcal{D} / \partial\mpliernode{i} = \energybound{i} - (\listenfrac{i} \listencost{i} + \xmitfrac{i} \xmitcost{i}),
\end{equation}
which is the difference between the power budget $\energybound{i}$ and the average power consumption of node $i$. Therefore, the dual can be minimized by using a gradient descent algorithm with inputs of step size $\stepsize_k > 0$, $\energyboundvec$, $\listencostvec$, and $\xmitcostvec$, which generates a state probability $\steadystatevec(k) ~(k = 1,2,\cdots)$. This algorithm is described in Algorithm~\ref{alg:gradient-descent} along with the following equations
%%
\begin{align}
\label{eqn:update-lm}
& \hspace{-0.1in} \mpliernode{i}(k) = \left[ \mpliernode{i}(k-1) - \stepsize_k (\energybound{i} - \listenfrac{i}(k) \listencost{i} - \xmitfrac{i}(k) \xmitcost{i}) \right]^+, \\
\label{eqn:compute-frac}
& \hspace{-0.1in} \listenfrac{i}(k) = \sum\nolimits_{\statevec \in \statespace_i^L} \steadystate_{\statevec}^{\mpliervec(k)}, ~\xmitfrac{i}(k) = \sum\nolimits_{\statevec \in \statespace_i^X} \steadystate_{\statevec}^{\mpliervec(k)}.
\end{align}
%%
Hence, with the right choice of step size $\stepsize_k$ (e.g., $\stepsize_k=1/k$), $\steadystatevec(k)$ converges to the optimal solution to {\namecp}.

%%
\subsection{Proof of Convergence}
% how the gradient descent algorithm relates to the protocol
Finally, to arrive at a distributed solution, instead of computing the quantities $\listenfrac{i}$ and $\xmitfrac{i}$ directly according to (\ref{eqn:compute-frac}) (which is centralized with high complexity), we can approximate the difference between the power budget and the average power consumption~\eqref{eq:gradient1} by observing the dynamics of the energy storage level at each node.
Specifically, each node $i$ can update its Lagrange multiplier $\mpliernode{i}(k)$ based on the difference between its energy storage levels at the end and the start of an interval of length $\epoch_{k}$, divided by $\epoch_{k}$, as described by (\ref{eqn:update-lm-epoch}). Therefore $\mpliernode{i}$ is updated according to a ``noisy'' gradient descent.
However, it follows from stochastic approximation (with Markov modulated noise) that by choosing step sizes and interval lengths as given in Theorem~\ref{thm:convergence}, these noisy updates will converge to $\mpliervec^*$ as $k \to \infty$ (see e.g., Theorem~1 of~\cite{jiang2009convergence}).
As mentioned in Section~\ref{ssec:distributed-param-choice}, the choice of parameters $\oursigma$, $\stepsize_{k}$, and $\epoch_{k}$ will affect the tradeoff between convergence time and the performance of {\name}. 

The detailed proof uses similar techniques as in the proof of Theorem 1 in~\cite{jiang2009convergence} with minor modifications.

%% notations of the proof

We use the same notation described in Section~\ref{ssec:proof-part-1}. Moreover, we have the following notation. We let $\numstate = \onenorm{\statespace}$ denote the total number of network states. Recall that each interval $k$ ($k = 1, 2, \cdots$) starts at time $t_{k-1}$ and ends at time $t_k$, and $t_0=0$. The Lagrangian multiplier $\mpliervec(k)$ is updated at the end of the $k$-th interval. The $k$-th interval is of the length $\epoch_{k} = t_{k} - t_{k-1}$. At time $t$, the probability of the system being in state $\statevec$ is denoted by $\networkprob_{\statevec}(t)$. Notice that throughout the $k$-th interval, $\mpliervec(k-1)$ remains changed and is updated at each node $i$ at time $t_{k}$ according to
%%
\begin{align}
\label{eqn:proof-update-lm-emp}
\mplier_{i}(k) = [ \mplier_{i}(k-1) - \stepsize_{k} ( \powerharv_{i} - \powerconsemp_{i}(k) ) ]^+,
\end{align}
%%
in which $\powerconsemp_i(k)$ is the \textit{empirical} energy consumption rate of node $i$ in the $k$-th interval.\footnote{Although we assume a constant power budget of $\powerharv_i$ at each node $i$, the proof can be easily extended to scenarios where $\powerharv_i$ varies with time.} The empirical energy consumption rate is given by
%%
\begin{align*}
\powerconsemp_i(k) & = \textstyle \int_{t_{k-1}}^{t_{k}} ( \listencost{i} \prob \left\{ \state_i(t) = l \right\} + \xmitcost{i} \prob \left\{ \state_i(t) = x \right\} )\, \textrm{d}t / \epoch_{k}, \\
& := \listencost{i} \cdot \listenfracemp{i}(k) + \xmitcost{i} \cdot \xmitfracemp{i}(k),
% & = \frac{1}{\epoch_{k}} \int_{t_{k-1}}^{t_{k}} [ \listencost{i} \cdot \nu_{\state_i=l}(t) + \xmitcost{i} \cdot \nu_{\state_i=x}(t) ]\, \textrm{d}t,
\end{align*}
%%
in which $\listenfracemp{i}(k)$ and $\xmitfracemp{i}(k)$ are the empirical fractions of time node $i$ spend in listen and transmit states, in the $k$-th interval. The relationship between the empirical energy consumption rate and the energy storage level (or battery values) $\bat_{i}(t)$ of node $i$ is given by $\powerharv_{i} - \powerconsemp_{i}(k) = [ \bat_{i}(t_{k}) - \bat_{i}(t_{k-1}) ] / \epoch_{k}$.
% ,which can be simply obtained from reading the energy storage levels.

In addition, let $\statevec^0(k)$ denote the state of the network Markov chain at the beginning of the $k$-th interval (i.e., at time $t_{k-1}$). Define the random vector $\mathbf{U}(k-1) := [ \powerconsempvec(k-1), \mpliervec(k-1), \statevec^0(k-1) ]$. For $k \geq 1$, let $\markovhist_{k-1}$ be the $\sigma$-field generated by $\mathbf{U}(0), \mathbf{U}(1), \cdots, \mathbf{U}(k-1)$.

In the $k$-th interval, define the gradient vector as $\gradientvec(k) = [\gradient_i(k)]$ whose $i$-th element $\gradient_i(k) = \powerharv_i(k) - \powercons_i(k)$. Given vector $\mpliervec(k-1)$, $\gradientvec(k)$ is a gradient of $\mathcal{L}(\mpliervec)$ (recall that the dual problem of {\namecp} is $\min\nolimits_{\mpliervec \succeq \bm{0}} \mathcal{L}(\mpliervec)$). To find the optimal $\mpliervec^*$ that solves the dual problem, the ideal algorithm (i.e., Algorithm~\ref{alg:gradient-descent}) uses the accurate descent direction of the gradient $\gradientvec$. However, {\name} follows~\eqref{eqn:proof-update-lm-emp} and only has an empirical estimation $\gradientempvec(k) = [\gradientemp_i(k)]$ of $\gradientvec(k)$, in which $\gradientemp_i(k) = \powerharv_i - \powerconsemp_i(k)$. The ``error'' term is given by $\gradientvec^{\rm err}(k) = [\gradient_i^{\rm err}(k)]$ in which
%%
\begin{align}
\label{eqn:proof-gradient-err}
\gradient_i^{\rm err}(k) & = \expectation{\gradientemp_i(k) | \markovhist_{k-1}} - \gradient_i(k) \powercons_i(k) - \expectation{ \powerconsemp_i(k) | \markovhist_{k-1} },
\end{align}
%%
The ``noise'' term is given by $\gradientvec^{\rm noise}(k) = [\gradient_i^{\rm noise}(k)]$ with
%%
\begin{align}
\label{eqn:proof-gradient-noise}
& \gradient_i^{\rm noise}(k) = \expectation{ \powerconsemp_i(k) | \markovhist_{k-1} } -  \powerconsemp_i(k).
\end{align}
%%
Therefore we can write the empirical gradient as
%%
\begin{align*}
\gradientemp_i(k) = \gradient_i(k) + \gradient_i^{\rm err}(k) + \gradient_i^{\rm noise}(k), ~\forall i \in \setnodes.
\end{align*}
%%
Notice that since $\powerharv_i(k)$ and $\powerconsemp_i(k)$ are both bounded, therefore the noise term is also bounded by some constant, i.e.,
%%
\begin{align*}
\onenorm{\gradient_i^{\rm noise}(k)} \leq \gradientmax^{\rm noise}, ~\forall i \in \setnode.
\end{align*}
%%

We first show that with {\name}, the error term $\gradientvec^{\rm err}(k)$~\eqref{eqn:proof-gradient-err} decreases ``fast enough'' with time. Then, we show that $\mpliervec$ converge to $\mpliervec^*$ with probability $1$ (w.p.$1$). We provide the detailed proof or part 1 below and the proof of part 2 is similar to the proof or Theorem 1 in~\cite{jiang2009convergence}.

%%
We assume that the step size $\stepsize_{k} > 0$ and the following conditions hold.
%%
\begin{align}
\label{eqn:proof-stepsize-constraint}
& \textstyle \sum\nolimits_{k=0}^{+\infty} \stepsize_{k} = +\infty, ~\sum\nolimits_{k=0}^{+\infty} \stepsize_{k}^{2} < +\infty \\
\label{eqn:proof-stepsize-constraint-2}
& \textstyle \sum\nolimits_{k=0}^{+\infty} \left( \stepsize_{k+1} \sum\nolimits_{m=1}^{k} \stepsize_{m} \right)^2 < +\infty, \\
\label{eqn:proof-aux-constraint} % auxiliary constraint
& \textstyle \sum\nolimits_{k=0}^{+\infty} \left[ \stepsize_{k+1} (\max\nolimits_{i} \mplier_{i}^{*} + \costmax 
\sum\nolimits_{m=1}^{k} \stepsize_{m}) f(k) / \epoch_{k+1} \right] < +\infty,
\end{align}
%%
in which, 
%%
\begin{align*}
& \textstyle \costmax = \max\nolimits_{i} \{ \max \{ \listencost{i}, \xmitcost{i} \} \}, \quad \xi_k = \costmax^{2} \sum\nolimits_{m=1}^{k} \stepsize_{m}, \\
& \textstyle f(k) = 2\numnode \costmax \numstate^{5/2} \cdot \exp ( 3\xi_{k} + \frac{5}{2} \numnode (\xi_k+1) ).
\end{align*}
%%
It can be easily verified that $\stepsize_{k} = 1/[(k+1)\log{(k+1)}]$ and $\epoch_{k} = k$ satisfy all the above conditions.


%%%%% BEGIN OF PROOF OF CONVERGENCE %%%%%

% proof of part 1: error term is decreasing fast enough
\noindent\textbf{Proof of Part 1}.
We drop the index $(k+1)$ and denote the Continuous-Time Markov chain (CTMC) in the $(k+1)$-th interval by $X(t),~\forall t \in [t_k, t_{k+1})$. For brevity, we assume $\oursigma=1$ and drop the term $1/\oursigma$. Recall from~\eqref{eqn:steady-state-prob}, $Z^{\mpliervec(k)}$ is a normalizing constant which can be bounded by
%%
\begin{align*}
Z^{\mpliervec(k)} & = \sum_{\statevec \in \statespace} \exp \left[ \tput_{\statevec} - \sum_{i \in \setnode_l(\statevec)} \mplier_i(k) \listencost{i} - \sum_{i \in \setnode_x(\statevec)} \mplier_i(k) \xmitcost{i} \right] \\
& \leq \numstate \cdot \exp{(\numnode)} = (2+\numnode) \cdot 2^{\numnode-1} \cdot \exp(\numnode),
\end{align*}
%%
in which the inequality comes from the fact that $\tput_{\statevec} \leq \numnode$. On the other hand, we also have
%%
\begin{align*}
& \exp \left[ \tput_{\statevec} - \sum\limits_{i \in \setnode_l(\statevec)} \mplier_i(k) \listencost{i} - \sum\limits_{i \in \setnode_x(\statevec)} \mplier_i(k) \xmitcost{i} \right] \\
& \quad \geq \exp [ - \numnode \cdot \costmax \cdot \max\limits_i \{ \mplier_i(k) \} ]
\end{align*}
%%
where $\costmax := \max\nolimits_{i \in \setnodes} \left\{ \max \left\{ \listencost{i}, \xmitcost{i} \right\} \right\}$. According to the updates of $\mpliervec(k)$, $\max\nolimits_i \{ \mplier_i(k) \}$ can be further bounded by $\max\nolimits_{i \in \setnodes} \{\mplier_{i}(k)\} \leq \costmax \cdot \sum\nolimits_{m=1}^{k} \stepsize_{m}$. Therefore, denoting $\xi_{k} := \costmax^{2} \cdot \sum\nolimits_{m=1}^{k} \stepsize_{m}$, we have the minimum probability in the stationary distribution lower bounded by
%%
\begin{align}
\label{eqn:proof-steadystate-min}
\steadystate_{\statevec}^{\mpliervec(k)} \geq \exp ( - \xi_{k} \numnode )  \left( \numstate \cdot \exp(\numnode) \right)^{-1} := \steadystate_{\rm min}^{\mpliervec(k)}.
\end{align}
%%

We first state the following useful proposition.

%% begin of prop
\begin{proposition}
Denote $\bm{Q} = [Q(\statevec, \statevec')]$ as the transition rate matrix of $X(t)$ in the $(k+1)$-th interval. If $Q(\statevec, \statevec') > 0$, there exists $Q_{\rm max} \geq Q_{\rm min} > 0$ such that
%%
\begin{align*}
Q_{k+1}^{\rm min} \leq Q(\statevec, \statevec') \leq Q_{k+1}^{\rm max}.
\end{align*}
%%
%In particular, $Q_{k+1}^{\rm max} := 2\numnode \exp(\xi_{k})$ and $Q_{k+1}^{\rm min} = \exp{(-\xi_{k})}$ are suffice.
%Furthermore, there is at most $2\numnode$ states $\statevec' \ne \statevec$ that can have positive transition rates $Q(\statevec, \statevec') > 0$.
\end{proposition}
%% end of prop
%% begin of proof
\begin{IEEEproof}
Given state $\statevec = [\state_i]$, there is a total number of $\numnode_s(\statevec) + 2\numnode_l(\statevec) + \numnode_x(\statevec) \leq 2\numnode$ states $\statevec'$ other than $\statevec$ that $X(t)$ can transition to. Recall that for any state $\statevec' \ne \statevec$, we have for each node $i$,
%%
\begin{align}
\label{eqn:trans-rate-matrix}
& Q(\statevec, \statevec') \nonumber \\
& = \left\{
\begin{aligned}
& \exp [ - \mplier_i(k) \listencost{i} ], && \state_i=s \to \state_i=l \\
& \exp [ \mplier_i(k) (\listencost{i} - \xmitcost{i}) ], && \state_i=l \to \state_i=x \\
& 1, && \state_i=l \to \state_i=s \\
& \exp( - \tput_{\statevec}), && \state_i=x \to \state_i=l
\end{aligned}
\right.
\end{align}
%%
It is easy to see that the transition rate is always bounded, and $Q_{k+1}^{\rm min} = \min\{ \exp(-\numnode), \exp(-\xi_k) \}$ will suffice. In particular, given the network size $\numnode$, for sufficiently large $k$, $\xi_k > \numnode$ holds, and therefore we use $Q_{k+1}^{\rm min} := \exp(-\xi_{k})$.

On the other hand, if for $\listencost{i} \leq \xmitcost{i}, \forall i \in \setnodes$, each one of the $2\numnode$ transition rates in~\eqref{eqn:trans-rate-matrix} is less than or equal to $1$, and $Q_{k+1}^{\rm max} = 2\numnode$ is sufficient. Second, if there exists some node $i$ such that $\listencost{i} > \xmitcost{i}$, beacause of the costs are always upper bounded by $\costmax$, the transition rate is also upper bounded by $\exp(\costmax \mpliermax) \leq \exp{(\costmax^{2} \sum\nolimits_{m=1}^{k} \stepsize_{m})} = \exp{(\xi_{k})}$. Therefore $Q_{k+1}^{\rm max} = 2\numnode \exp{(\xi_{k})}$ is sufficient.
\end{IEEEproof}
%% end of proof

Following the regular process, we first perform uniformization of the continuous time Markov chain $X(t)$. For the Markov chian $X(t)$, if each element of its transition rate matrix $\bm{Q}$ has an absolulte value less that a constant $Q_{k+1}^{\rm max}$, then we can write $X(t) = Y(M(t))$, in which $Y(n)$ is a discrete time Markov chain with probability transition matrix $\bm{P} = \bm{I} + \bm{Q} / Q_{k+1}^{\rm max}$ and $\bm{I}$ is the identity matrix. $M(t)$ is an independent Poisson process with rate $Q_{k+1}^{\rm max}$.
% Recall that $Q(\statevec, \statevec') > 0$ for {\it at most} $2\numnode$ different states $\statevec' \ne \statevec$. We have the following proposition which gives a value of $A_{k+1}$ that is sufficient for the uniformization.

% %% begin of prop
% \begin{proposition}
% The following value of $A_{k+1}$ is sufficient for the uniformization,
% %%
% \begin{align}
% \label{eqn:proof-uniformization-rate}
% A_{k+1} := 2\numnode \exp(\xi_{k}),
% \end{align}
% %%
% \end{proposition}
% %% end of prop
% %% proof of prop
% \begin{proof}
% First, if for $\listencost{i} \leq \xmitcost{i}, \forall i \in \setnodes$, each one of the $2\numnode$ transition rates in~\eqref{eqn:trans-rate-matrix} is less than or equal to $1$, and $A_{k+1} = 2\numnode$ is sufficient. Second, if there exists some node $i$ such that $\listencost{i} > \xmitcost{i}$, beacause of the costs are always upper bounded by $\costmax$, the transition rate is also upper bounded by $\exp(\costmax \mpliermax) \leq \exp{(\costmax^{2} \sum\nolimits_{m=1}^{k} \stepsize_{m})} = \exp{(\xi_{k})}$. Thus $A_{k+1} = 2\numnode \exp{(\xi_{k})}$ is sufficient. Since $\xi_{k} \geq 0$ holds, using $A_{k+1}$ defined as in (\ref{eqn:proof-uniformization-rate}), the uniformization is valid.
% \end{proof}
% %% end of proof

We estimate how far the empirical power consumption $\expectation{\powerconsemp_i(k+1) | \markovhist_k}$ is away from the desired value $\powercons_{i}(k+1)$ (under fixed $\mpliervec(k)$). Denote the probability of $X(t)$ in state $\statevec$ at time $t \in [t_{k}, t_{k+1})$ by $\networkprob_{\statevec}(t)$ and $\networkprobvec(t) = [\networkprob_{\statevec}(t)]$. Given the initial state at time $t_k$ is $\statevec^0(k+1)$, We have
%%
\begin{align*}
& \textstyle \expectation{ \powerconsemp_i(k+1) | \markovhist_k }\\
& \textstyle = \expectation{ \int_{t_k}^{t_{k+1}} \sum_{\statevec \in \statespace} \left( \mathbf{1}_{ 
\{\state_i = l\} } \listencost{i} +  \mathbf{1}_{ \{ \state_i = x \} } \xmitcost{i} \right)\, \textrm{d}t / \epoch_{k+1} } \\
& \textstyle = \int_{t_k}^{t_{k+1}} \sum_{\statevec \in \statespace} ( \prob \left\{ \state_i(t) = l \right\} \listencost{i} + \prob \left\{ \state_i(t) = x \right\} \xmitcost{i} )\, \textrm{d}t / \epoch_{k+1} \\
& \textstyle = \frac{\listencost{i}}{\epoch_{k+1}} \sum_{\statevec \in \statespace_i^l} \int_{t_k}^{t_{k+1}} \networkprob_{\statevec}(t)\, \textrm{d}t + \frac{\xmitcost{i}}{\epoch_{k+1}} \sum_{\statevec \in \statespace_i^x} \int_{t_{k}}^{t_{k+1}} \networkprob_{\statevec}(t)\, \textrm{d}t \\
& \textstyle = \listencost{i} \cdot \listenfracemp{i}(k+1) + \xmitcost{i} \cdot \xmitfracemp{i}(k+1),
\end{align*}
%%
in which
%%
\begin{align*}
& \textstyle \emplistenfrac{i}(k+1) = \sum\limits_{\statevec \in \statespace_i^l} \int_{t_{k}}^{t_{k+1}} \networkprob_{\statevec}(t) \, \textrm{d}t / \epoch_{k+1} \\
& \textstyle \xmitfracemp{i}(k+1) = \sum\limits_{\statevec \in \statespace_i^x} \int_{t_{k}}^{t_{k+1}} \networkprob_{\statevec}(t) \, \textrm{d}t / \epoch_{k+1}
\end{align*}
%%
are the empirical average probabilities that node $i$ spends in listen and transmit states in the $(k+1)$-th interval.

Let $\slev$ with $|\slev| \leq 1$ be the Second Largest Eigenvalue of the transition probability matrix $\bm{P} = \bm{I} + \bm{Q} / Q_{k+1}^{\rm max}$, and the total variation distance between $\networkprobvec(t)$ and $\steadystatevec^{\mpliervec(k)}$ can be bounded by
%%
\begin{align*}
\textstyle \normtv{\networkprobvec(t) - \steadystatevec^{\mpliervec(k)}} = \frac{1}{2} \sum\nolimits_{\statevec \in \statespace} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} }.
\end{align*}
%%
This total variation distance can be bounded by
%%
\begin{align}
\label{eqn:proof-norvtv-bound}  % total variance bound
\textstyle \normtv{\networkprobvec(t) - \steadystatevec^{\mpliervec(k)}}
& \textstyle = \frac{1}{2} \sum\nolimits_{\statevec \in \statespace} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} } \nonumber \\
& \textstyle \leq \frac{1}{2} \sqrt{ \frac{1 - \steadystate_{\statevec^{0}}^{\mpliervec(k)}}{\steadystate_{\statevec^{0}}^{\mpliervec(k)}} } \exp ( - Q_{k+1}^{\rm max} (1-\slev) t) \nonumber \\
& \textstyle \leq \frac{1}{2} \frac{1}{\sqrt{\steadystate_{\rm min}^{\mpliervec(k)}}} \exp ( - Q_{k+1}^{\rm max} (1-\slev) t). 
\end{align}
%%
Also, the Second Largest Eigenvalue, $\slev$, can be bounded by Cheeger's inequality~\cite{diaconis1991geometric}, i.e.,
%%
\begin{align*}
\slev \leq 1 - \phi^2 / 2 \Leftrightarrow 1 / (1-\theta_2) \leq 2 / \phi^2
\end{align*}
%%
where $\phi$ is the ``conductance'' of $\bm{P}$, which satisfies the following inequality
%%
\begin{align*}
\textstyle \phi & \geq \min_{\statevec \ne \statevec', P(\statevec, \statevec') > 0} \{  \steadystate_{\rm min}^{\mpliervec(k)} P(\statevec, \statevec') \} \geq \steadystate_{\rm min}^{\mpliervec(k)} \cdot Q_{k+1}^{\rm min} / Q_{k+1}^{\rm max}.
\end{align*}
%%
Therefore we obtain
%%
\begin{align}
\label{eqn:proof-slev-bound}
\frac{1}{1-\slev} \leq \frac{2}{\phi^2} \leq 2 \left( \frac{Q_{k+1}^{\rm max}}{ \steadystate_{\rm min}^{\mpliervec(k)} \cdot Q_{k+1}^{\rm min}} \right)^{2}.
\end{align}
%%

Putting everything back into the estimation, we have
%%
\begin{align*}
& \onenorm{ \expectation{ \powerconsemp_i(k+1) | \markovhist_k } - \powercons_i(k+1)} \\
& = \onenorm{ \listencost{i} (\listenfracemp{i}(k+1) - \listenfrac{i}(k+1)) + \xmitcost{i} (\xmitfracemp{i}(k+1) - \xmitfrac{i}(k+1)) } \\
& \leq \listencost{i} \onenorm{ \listenfracemp{i}(k+1) - \listenfrac{i}(k+1) } + \xmitcost{i} \onenorm{ \xmitfracemp{i}(k+1) - \xmitfrac{i}(k+1) }.
% & \leq \costmax \cdot \normtv{ \bar{\mu} - \steadystate(\mpliervec(k))},
\end{align*}
%%
Furthermore, we have
%%
\begin{align*}
& \textstyle \onenorm{ \listenfracemp{i}(k+1) - \listenfrac{i}(k+1) } \\
& \textstyle  = \onenorm{ \sum\nolimits_{\statevec \in \statespace_i^l} \int_{t_{k}}^{t_{k+1}} ( \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} ) \, \textrm{d}t / \epoch_{k+1} } \\
% & \leq \sum\limits_{\statevec \in \statespace_i^l} \int_{t_{k}}^{t_{k+1}} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} } \, \textrm{d}t / \epoch_{k+1} \\
& \textstyle \leq \int_{t_{k}}^{t_{k+1}} \sum\nolimits_{\statevec \in \statespace_i^l} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} } \, \textrm{d}t / \epoch_{k+1}.
\end{align*}
%%
Similarly,
%%
\begin{align*}
& \textstyle \onenorm{ \xmitfracemp{i}(k+1) - \xmitfrac{i}(k+1) } \\
& \textstyle \leq \int_{t_{k}}^{t_{k+1}} \sum\nolimits_{\statevec \in \statespace_i^x} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} } \, \textrm{d}t / \epoch_{k+1}.
\end{align*}
%%
Adding both terms together we obtain
%%
\begin{align*}
& \textstyle \listencost{i} \onenorm{ \listenfracemp{i}(k+1) - \listenfrac{i}(k+1) } + \xmitcost{i} \onenorm{ \xmitfracemp{i}(k+1) - \xmitfrac{i}(k+1) } \\
& \textstyle \leq \costmax \int_{t_k}^{t_{k+1}} \sum\nolimits_{\statevec \in \statespace} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} } \, \textrm{d}t / \epoch_{k+1} \\
& \textstyle \leq \frac{\costmax}{\sqrt{\steadystate_{\rm min}^{\mpliervec(k)}}} \int_{t_k}^{t_{k+1}} \exp{(-Q_{k+1}^{\rm max}(1-\slev)t)} \, \textrm{d}t / \epoch_{k+1} ~\textrm{(use~\eqref{eqn:proof-norvtv-bound})} \\
& \textstyle \leq \frac{\costmax}{\sqrt{\steadystate_{\rm min}^{\mpliervec(k)}}} \int_{0}^{t_{k+1}} \exp{(-Q_{k+1}^{\rm max}(1-\slev)t)} \, \textrm{d}t / \epoch_{k+1} \\
& \textstyle \leq \frac{\costmax}{\sqrt{\steadystate_{\rm min}^{\mpliervec(k)}}} \cdot \left[ 2 Q_{k+1}^{\rm max} (1-\slev) \right]^{-1} / \epoch_{k+1} \\
& \textstyle \leq \frac{\costmax Q_{k+1}^{\rm max}}{ \epoch_{k+1} (Q_{k+1}^{\rm min})^2 (\steadystate_{\rm min}^{\mpliervec(k)})^{5/2} }
:= f(k) / \epoch_{k+1}, ~\textrm{(use~\eqref{eqn:proof-slev-bound})}
\end{align*}
%%
in which $f(k) := \frac{\costmax Q_{k+1}^{\rm max}}{ (Q_{k+1}^{\rm min})^2 (\steadystate_{\rm min}^{\mpliervec(k)})^{5/2} }$.
%%
Therefore we have,
%%
\begin{align*}
\onenorm{ \expectation{ \powerconsemp_i(k+1) | \markovhist_k } - \powercons_i(\mpliervec(k)) } \leq f(k) / \epoch_{k+1},
\end{align*}
%%
%%
and the error term, defined in~\eqref{eqn:proof-gradient-err}, satisfies $\onenorm{ \gradient_i^{\rm err}(k+1)} \leq f(k) / \epoch_{k+1}$. Therefore, with defined $f(k)$ and proper choice of $\epoch_{k+1}$ (e.g., $\epoch_{k+1} = k+1$), the error term is diminishing.


% Since $\onenorm{\mplier_i(k) - \mplier_k^*} \leq \max\nolimits_{i} \mplier_i^* + \costmax \sum\nolimits_{m=1}^k \stepsize_{m}$, we can show that the term $(\mpliervec(k) - \mpliervec^*(k))^T \cdot \gradientvec^{\rm err}(k+1)$ is diminishing:
% %%
% \begin{align}
% \label{eqn:proof-gradient-error-bound}
% & \sum\limits_{k=0}^{+\infty} \left( \stepsize_{k+1} \onenorm{ ( \mpliervec(k) - \mpliervec^* )^{T} \cdot \gradientvec^{\rm err}(k+1) } \right) \nonumber \\
% & \leq \numnode \sum\limits_{k=0}^{+\infty} [ \stepsize_{k+1} (\max\limits_{i} \mplier_i^* + \costmax \sum\limits_{m=1}^k \stepsize_{m}) f(k) / \epoch_{k+1} ] \nonumber \\
% % & = \numnode \costmax \cdot \sum\limits_{k=0}^{+\infty} [ \stepsize_{k+1} \cdot ( \sum\limits_{k'=1}^k \stepsize_{k'}) \cdot f(k) / \epoch_{k+1} ] \nonumber \\
% % & \quad~ + \numnode \costmax \cdot \max\limits_{i} \mplier_i^* \cdot \sum\limits_{k=0}^{+\infty} [ \stepsize_{k+1} \cdot f(k) / \epoch_{k+1} ]
% & < +\infty
% \end{align}
% where the last inequality comes from the condition~\eqref{eqn:proof-aux-constraint}.
% %%


%%
\noindent\textbf{Proof of Part 2}.
The main results of this part is summarized in the following lemma, and the proof is similar to the proof of Theorem~1 in\cite{jiang2009convergence}.
%% begin of lemma
\begin{mylemma}
If~\eqref{eqn:proof-stepsize-constraint-2} and~\eqref{eqn:proof-aux-constraint} hold, then with {\name}, $\mpliervec$ converges to $\mpliervec^*$ with probability 1.
\end{mylemma}
%% end of lemma

Combining Part 1 and Part 2, we complete the proof of Theorem~\ref{thm:convergence}.  \hfill $\Box$

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../conext16"
%%% End:


==> tex/aux_gen_impl_tput_fig.tex <==
% separate plots
\begin{figure*}[!htb]
\centering
\hspace{-0.10in} 
\includegraphics[width=0.52\columnwidth]{figs/eval_figs/eval_tput_bat_P_1_N_5.eps} \includegraphics[width=0.52\columnwidth]{figs/eval_figs/eval_tput_bat_P_1_N_10.eps}
\includegraphics[width=0.52\columnwidth]{figs/eval_figs/eval_tput_bat_P_5_N_5.eps} \includegraphics[width=0.52\columnwidth]{figs/eval_figs/eval_tput_bat_P_5_N_10.eps}
\vspace{-0.5\baselineskip}
\caption{Points marked as ``Ideal'' (``Relaxed'') represent ratio of experimental throughput normalized to the achievable throughput obtained by using the target power budget (actual power consumption) and points marked as ``Battery Variance'' present the average, minimum, and maximum ratios of power consumption normalized to target power budget, with $\numnode \in \{5, 10\}$, $\energybound{} \in \{ \ourmW{1}, \ourmW{5} \}$, and $\oursigma \in \{0.25, 0.5\}$.}
\label{fig:impl-tput}
\vspace{-1\baselineskip}
\end{figure*}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> tex/proof_convergence_short_v0.tex <==
\section{Detailed Proof of Theorem 1}
\label{append:proof-convergence}

The proof of Theorem~\ref{thm:convergence} uses similar techniques as in the proof of Theorem 1 in~\cite{jiang2009convergence} with minor modifications.

%% notations of the proof
\subsection{Some Notation}
We use the same notation described in Appendix~\ref{append:proof-dbe}. Moreover, we have the following notation. We let $\numstate = \onenorm{\statespace}$ denote the total number of network states. Recall that each interval $k$ ($k = 1, 2, \cdots$) starts at time $t_{k-1}$ and ends at time $t_k$, and $t_0=0$. The Lagrangian multiplier $\mpliervec(k)$ is updated at the end of the $k$-th interval. The $k$-th interval is of the length $\epoch_{k} = t_{k} - t_{k-1}$. At time $t$, the probability of the system being in state $\statevec$ is denoted by $\networkprob_{\statevec}(t)$. Notice that throughout the $k$-th interval, $\mpliervec(k-1)$ remains changed and is updated at each node $i$ at time $t_{k}$ according to
%%
\begin{align}
\label{eqn:proof-update-lm-emp}
\mplier_{i}(k) = [ \mplier_{i}(k-1) - \stepsize_{k} ( \powerharv_{i} - \powerconsemp_{i}(k) ) ]^+,
\end{align}
%%
in which $\powerconsemp_i(k)$ is the \textit{empirical} energy consumption rate of node $i$ in the $k$-th interval.\footnote{Although we assume a constant power budget of $\powerharv_i$ at each node $i$, the proof can be easily extended to scenarios where $\powerharv_i$ varies with time.} The empirical energy consumption rate is given by
%%
\begin{align*}
\powerconsemp_i(k) & = \int_{t_{k-1}}^{t_{k}} ( \listencost{i} \prob \left\{ \state_i(t) = l \right\} + \xmitcost{i} \prob \left\{ \state_i(t) = x \right\} )\, \textrm{d}t / \epoch_{k}, \\
& := \listencost{i} \cdot \listenfracemp{i}(k) + \xmitcost{i} \cdot \xmitfracemp{i}(k),
% & = \frac{1}{\epoch_{k}} \int_{t_{k-1}}^{t_{k}} [ \listencost{i} \cdot \nu_{\state_i=l}(t) + \xmitcost{i} \cdot \nu_{\state_i=x}(t) ]\, \textrm{d}t,
\end{align*}
%%
in which $\listenfracemp{i}(k)$ and $\xmitfracemp{i}(k)$ are the empirical fractions of time node $i$ spend in listen and transmit states, in the $k$-th interval. The relationship between the empirical energy consumption rate and the energy storage levels (or battery values) of node $i$, $\bat_i(t)$, is given by $\powerharv_{i} - \powerconsemp_{i}(k) = [ \bat_{i}(t_{k}) - \bat_{i}(t_{k-1}) ] / \epoch_{k}$,
which can be simply obtained from reading the energy storage levels.

In addition, let $\statevec^0(k)$ denote the state of the network Markov chain at the beginning of the $k$-th interval (i.e., at time $t_{k-1}$). Define the random vector $\mathbf{U}(k-1) := [ \powerconsempvec(k-1), \mpliervec(k-1), \statevec^0(k-1) ]$. For $k \geq 1$, let $\markovhist_{k-1}$ be the $\sigma$-field generated by $\mathbf{U}(0), \mathbf{U}(1), \cdots, \mathbf{U}(k-1)$.

In the $k$-th interval, define the gradient vector as $\gradientvec(k) = [\gradient_i(k)]$ whose $i$-th element $\gradient_i(k) = \powerharv_i(k) - \powercons_i(k)$. Given vector $\mpliervec(k-1)$, $\gradientvec(k)$ is a gradient of $\mathcal{L}(\mpliervec)$ (recall that the dual problem of {\namecp} is $\min\nolimits_{\mpliervec \succeq \bm{0}} \mathcal{L}(\mpliervec)$). To find the optimal $\mpliervec^*$ that solves the dual problem, the ideal algorithm (i.e., Algorithm~\ref{alg:gradient-descent}) uses the accurate descent direction of the gradient $\gradientvec$. However, {\name} follows~\eqref{eqn:proof-update-lm-emp} and only has an empirical estimation of $\gradientvec(k)$, denoted by $\gradientempvec(k) = [\gradientemp_i(k)]$, in which $\gradientemp_i(k) = \powerharv_i - \powerconsemp_i(k)$. The ``error'' term is given by $\gradientvec^{\rm err}(k) = [\gradient_i^{\rm err}(k)]$ in which
%%
\begin{align}
\label{eqn:proof-gradient-err}
\gradient_i^{\rm err}(k) & = \expectation{\gradientemp_i(k) | \markovhist_{k-1}} - \gradient_i(k) \nonumber \\
& = \powercons_i(k) - \expectation{ \powerconsemp_i(k) | \markovhist_{k-1} },
\end{align}
%%
The ``noise'' term is given by $\gradientvec^{\rm noise}(k) = [\gradient_i^{\rm noise}(k)]$ with
%%
\begin{align}
\label{eqn:proof-gradient-noise}
& \gradient_i^{\rm noise}(k) = \expectation{ \powerconsemp_i(k) | \markovhist_{k-1} } -  \powerconsemp_i(k).
\end{align}
%%
Therefore we can write the empirical gradient as
%%
\begin{align*}
\gradientemp_i(k) = \gradient_i(k) + \gradient_i^{\rm err}(k) + \gradient_i^{\rm noise}(k), ~\forall i \in \setnodes.
\end{align*}
%%
Notice that since $\powerharv_i(k)$ and $\powerconsemp_i(k)$ are both bounded, therefore the noise term is also bounded by some constant, i.e.,
%%
\begin{align*}
\onenorm{\gradient_i^{\rm noise}(k)} \leq \gradientmax^{\rm noise}, ~\forall i \in \setnode.
\end{align*}
%%

\subsection{Proof of Convergence}
% summary of proof
The proof is composed of two parts. In part 1, we show that with {\name}, the error term $\gradientvec^{\rm err}(k)$~\eqref{eqn:proof-gradient-err} decreases ``fast enough'' with time. In part 2, we show that $\mpliervec$ converge to $\mpliervec^*$ with probability $1$ (w.p.$1$). We provide the detailed proof or part 1 below and the proof of part 2 is similar to the proof or Theorem 1 in~\cite{jiang2009convergence}.

%%
We assume that the step size $\stepsize_{k} > 0$ and the following conditions hold.
%%
\begin{align}
\label{eqn:proof-stepsize-constraint}
& \sum\limits_{k=0}^{+\infty} \stepsize_{k} = +\infty, ~\sum\limits_{k=0}^{+\infty} \stepsize_{k}^{2} < +\infty \\
\label{eqn:proof-stepsize-constraint-2}
& \sum\limits_{k=0}^{+\infty} \left( \stepsize_{k+1} \sum\limits_{m=1}^{k} \stepsize_{m} \right)^2 < +\infty, \\
\label{eqn:proof-aux-constraint} % auxiliary constraint
& \sum\limits_{k=0}^{+\infty} \left[ \stepsize_{k+1} (\max\limits_{i} \mplier_{i}^{*} + \costmax 
\sum\limits_{m=1}^{k} \stepsize_{m}) f(k) / \epoch_{k+1} \right] < +\infty,
\end{align}
%%
in which, 
%%
\begin{align*}
& \costmax = \max\limits_{i} \{ \max \{ \listencost{i}, \xmitcost{i} \} \}, \quad \xi_k = \costmax^{2} \sum\limits_{m=1}^{k} \stepsize_{m}, \\
& f(k) = 2\numnode \costmax \numstate^{5/2} \cdot \exp ( 3\xi_{k} + \frac{5}{2} \numnode (\xi_k+1) ).
\end{align*}
%%
It can be easily verified that $\stepsize_{k} = 1/[(k+1)\log{(k+1)}]$ and $\epoch_{k} = k$ satisfy all the above conditions.


%%%%% BEGIN OF PROOF OF CONVERGENCE %%%%%

% proof of part 1: error term is decreasing fast enough
\noindent\textbf{Proof of Part 1}.
We drop the index $(k+1)$ and denote the Continuous-Time Markov chain (CTMC) in the $(k+1)$-th interval by $X(t),~\forall t \in [t_k, t_{k+1})$. For brevity, we assume $\oursigma=1$ and drop the term $1/\oursigma$. From~\eqref{eqn:steady-state-prob}, the {\em steady state distribution} of $X(t)$ with given $\mpliervec(k)$ is given by
%%
\begin{align*}
\steadystate_{\statevec}^{\mpliervec(k)} = \exp [ \tput_{\statevec} - \sum\limits_{i \in \setnode_l(\statevec)} \mplier_i(k) \listencost{i} - \sum\limits_{i \in \setnode_x(\statevec)} \mplier_i(k) \xmitcost{i} ] / Z^{\mpliervec(k)}
\end{align*}
%%
where $Z^{\mpliervec(k)}$ is a constant such that $\sum_{\statevec \in \statespace} \steadystate_{\statevec}^{\mpliervec(k)} = 1$. This constant can be bounded by
%%
\begin{align*}
& \sum_{\statevec \in \statespace} \exp \left[ \tput_{\statevec} - \sum_{i \in \setnode_l(\statevec)} \mplier_i(k) \listencost{i} - \sum_{i \in \setnode_x(\statevec)} \mplier_i(k) \xmitcost{i} \right] \\
& \quad \leq \numstate \cdot \exp{(\numnode)} = (2+\numnode) \cdot 2^{\numnode-1} \cdot \exp(\numnode),
\end{align*}
%%
in which the inequality comes from the fact that $\tput_{\statevec} \leq \numnode$. On the other hand, we also have
%%
\begin{align*}
& \exp \left[ \tput_{\statevec} - \sum\limits_{i \in \setnode_l(\statevec)} \mplier_i(k) \listencost{i} - \sum\limits_{i \in \setnode_x(\statevec)} \mplier_i(k) \xmitcost{i} \right] \\
& \quad \geq \exp [ - \numnode \cdot \costmax \cdot \max\limits_i \{ \mplier_i(k) \} ]
\end{align*}
%%
where $\costmax := \max\nolimits_{i \in \setnodes} \left\{ \max \left\{ \listencost{i}, \xmitcost{i} \right\} \right\}$. According to the updates of $\mpliervec(k)$, $\max\nolimits_i \{ \mplier_i(k) \}$ can be further bounded by $\max\nolimits_{i \in \setnodes} \{\mplier_{i}(k)\} \leq \costmax \cdot \sum\nolimits_{m=1}^{k} \stepsize_{m}$. Therefore, denoting $\xi_{k} := \costmax^{2} \cdot \sum\nolimits_{m=1}^{k} \stepsize_{m}$, we have the minimum probability in the stationary distribution lower bounded by
%%
\begin{align}
\label{eqn:proof-steadystate-min}
\steadystate_{\statevec}^{\mpliervec(k)} \geq \frac{\exp ( - \xi_{k} \numnode )}{ \numstate \cdot \exp(\numnode)} := \steadystate_{\rm min}^{\mpliervec(k)}.
\end{align}
%%

Before proceeding with the proof, we first state the following useful propositions.

%% begin of prop
\begin{proposition}
Denote $\bm{Q} = [Q(\statevec, \statevec')]$ as the transition rate matrix of $X(t)$ in the $(k+1)$-th interval. If $Q(\statevec, \statevec') > 0$, there exists $Q_{\rm max} \geq Q_{\rm min} > 0$ such that
%%
\begin{align*}
Q_{k+1}^{\rm min} \leq Q(\statevec, \statevec') \leq Q_{k+1}^{\rm max}.
\end{align*}
%%
%In particular, $Q_{k+1}^{\rm max} := 2\numnode \exp(\xi_{k})$ and $Q_{k+1}^{\rm min} = \exp{(-\xi_{k})}$ are suffice.
%Furthermore, there is at most $2\numnode$ states $\statevec' \ne \statevec$ that can have positive transition rates $Q(\statevec, \statevec') > 0$.
\end{proposition}
%% end of prop
%% begin of proof
\begin{proof}
Given state $\statevec = [\state_i]$, there is a total number of $\numnode_s(\statevec) + 2\numnode_l(\statevec) + \numnode_x(\statevec) \leq 2\numnode$ states $\statevec'$ other than $\statevec$ that $X(t)$ can transition to. Recall that for any state $\statevec' \ne \statevec$, we have for each node $i$,
%%
\begin{align}
\label{eqn:trans-rate-matrix}
& Q(\statevec, \statevec') \nonumber \\
& = \left\{
\begin{aligned}
& \exp [ - \mplier_i(k) \listencost{i} ], && \state_i=s \to \state_i=l \\
& \exp [ \mplier_i(k) (\listencost{i} - \xmitcost{i}) ], && \state_i=l \to \state_i=x \\
& 1, && \state_i=l \to \state_i=s \\
& \exp( - \tput_{\statevec}),. && \state_i=x \to \state_i=l
\end{aligned}
\right.
\end{align}
%%
It is easy to see that the transition rate is always bounded, and $Q_{k+1}^{\rm min} = \min\{ \exp(-\numnode), \exp(-\xi_k) \}$ will suffice. In particular, given the network size $\numnode$, for sufficiently large $k$, $\xi_k > \numnode$ holds, and therefore we use $Q_{k+1}^{\rm min} := \exp(-\xi_{k})$.

On the other hand, if for $\listencost{i} \leq \xmitcost{i}, \forall i \in \setnodes$, each one of the $2\numnode$ transition rates in~\eqref{eqn:trans-rate-matrix} is less than or equal to $1$, and $Q_{k+1}^{\rm max} = 2\numnode$ is sufficient. Second, if there exists some node $i$ such that $\listencost{i} > \xmitcost{i}$, beacause of the costs are always upper bounded by $\costmax$, the transition rate is also upper bounded by $\exp(\costmax \mpliermax) \leq \exp{(\costmax^{2} \sum\nolimits_{m=1}^{k} \stepsize_{m})} = \exp{(\xi_{k})}$. Therefore $Q_{k+1}^{\rm max} = 2\numnode \exp{(\xi_{k})}$ is sufficient.
\end{proof}
%% end of proof

Following the regular process, we first perform uniformization of the continuous time Markov chain $X(t)$. For the Markov chian $X(t)$, if each element of its transition rate matrix $\bm{Q}$ has an absolulte value less that a constant $Q_{k+1}^{\rm max}$, then we can write $X(t) = Y(M(t))$, in which $Y(n)$ is a discrete time Markov chain with probability transition matrix $\bm{P} = \bm{I} + \bm{Q} / Q_{k+1}^{\rm max}$ and $\bm{I}$ is the identity matrix. $M(t)$ is an independent Poisson process with rate $Q_{k+1}^{\rm max}$.
% Recall that $Q(\statevec, \statevec') > 0$ for {\it at most} $2\numnode$ different states $\statevec' \ne \statevec$. We have the following proposition which gives a value of $A_{k+1}$ that is sufficient for the uniformization.

% %% begin of prop
% \begin{proposition}
% The following value of $A_{k+1}$ is sufficient for the uniformization,
% %%
% \begin{align}
% \label{eqn:proof-uniformization-rate}
% A_{k+1} := 2\numnode \exp(\xi_{k}),
% \end{align}
% %%
% \end{proposition}
% %% end of prop
% %% proof of prop
% \begin{proof}
% First, if for $\listencost{i} \leq \xmitcost{i}, \forall i \in \setnodes$, each one of the $2\numnode$ transition rates in~\eqref{eqn:trans-rate-matrix} is less than or equal to $1$, and $A_{k+1} = 2\numnode$ is sufficient. Second, if there exists some node $i$ such that $\listencost{i} > \xmitcost{i}$, beacause of the costs are always upper bounded by $\costmax$, the transition rate is also upper bounded by $\exp(\costmax \mpliermax) \leq \exp{(\costmax^{2} \sum\nolimits_{m=1}^{k} \stepsize_{m})} = \exp{(\xi_{k})}$. Thus $A_{k+1} = 2\numnode \exp{(\xi_{k})}$ is sufficient. Since $\xi_{k} \geq 0$ holds, using $A_{k+1}$ defined as in (\ref{eqn:proof-uniformization-rate}), the uniformization is valid.
% \end{proof}
% %% end of proof

We estimate how far the empirical power consumption $\expectation{\powerconsemp_i(k+1) | \markovhist_k}$ is away from the desired value $\powercons_{i}(k+1)$ (under fixed $\mpliervec(k)$). Denote the probability of $X(t)$ in state $\statevec$ at time $t \in [t_{k}, t_{k+1})$ by $\networkprob_{\statevec}(t)$ and $\networkprobvec(t) = [\networkprob_{\statevec}(t)]$. Given the initial state at time $t_k$ is $\statevec^0(k+1)$, We have
%%
\begin{align*}
& \expectation{ \powerconsemp_i(k+1) | \markovhist_k }\\
& = \expectation{ \int_{t_k}^{t_{k+1}} \sum_{\statevec \in \statespace} \left( \mathbf{1}_{ 
\{\state_i = l\} } \listencost{i} +  \mathbf{1}_{ \{ \state_i = x \} } \xmitcost{i} \right)\, \textrm{d}t / \epoch_{k+1} } \\
& = \int_{t_k}^{t_{k+1}} \sum_{\statevec \in \statespace} ( \prob \left\{ \state_i(t) = l \right\} \listencost{i} + \prob \left\{ \state_i(t) = x \right\} \xmitcost{i} )\, \textrm{d}t / \epoch_{k+1} \\
& = \frac{\listencost{i}}{\epoch_{k+1}} \sum_{\statevec \in \statespace_i^l} \int_{t_k}^{t_{k+1}} \networkprob_{\statevec}(t)\, \textrm{d}t + \frac{\xmitcost{i}}{\epoch_{k+1}} \sum_{\statevec \in \statespace_i^x} \int_{t_{k}}^{t_{k+1}} \networkprob_{\statevec}(t)\, \textrm{d}t \\
& = \listencost{i} \cdot \listenfracemp{i}(k+1) + \xmitcost{i} \cdot \xmitfracemp{i}(k+1),
\end{align*}
%%
in which
%%
\begin{align*}
& \emplistenfrac{i}(k+1) = \sum\limits_{\statevec \in \statespace_i^l} \int_{t_{k}}^{t_{k+1}} \networkprob_{\statevec}(t) \, \textrm{d}t / \epoch_{k+1} \\
& \xmitfracemp{i}(k+1) = \sum\limits_{\statevec \in \statespace_i^x} \int_{t_{k}}^{t_{k+1}} \networkprob_{\statevec}(t) \, \textrm{d}t / \epoch_{k+1}
\end{align*}
%%
are the empirical average probabilities that node $i$ spends in listen and transmit states in the $(k+1)$-th interval.

Let $\slev$ with $|\slev| \leq 1$ be the Second Largest Eigenvalue of the transition probability matrix $\bm{P} = \bm{I} + \bm{Q} / Q_{k+1}^{\rm max}$, and define the total variation distance by $\norm{\cdot}_{\rm TV}$, i.e.,
%%
\begin{align*}
\normtv{\networkprobvec(t) - \steadystatevec^{\mpliervec(k)}} = \frac{1}{2} \sum\limits_{\statevec \in \statespace} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} }.
\end{align*}
%%
This total variation distance can be bounded by
%%
\begin{align}
\label{eqn:proof-norvtv-bound}  % total variance bound
\normtv{\networkprobvec(t) - \steadystatevec^{\mpliervec(k)}}
& \leq \frac{1}{2} \sqrt{ \frac{1 - \steadystate_{\statevec^{0}}^{\mpliervec(k)}}{\steadystate_{\statevec^{0}}^{\mpliervec(k)}} } \exp ( - Q_{k+1}^{\rm max} (1-\slev) t) \nonumber \\
& \leq \frac{1}{2} \frac{1}{\sqrt{\steadystate_{\rm min}^{\mpliervec(k)}}} \exp ( - Q_{k+1}^{\rm max} (1-\slev) t). 
\end{align}
%%
Also, the Second Largest Eigenvalue, $\slev$, can be bounded by Cheeger's inequality~\cite{diaconis1991geometric}, i.e.,
%%
\begin{align*}
\slev \leq 1 - \frac{\phi^2}{2} \Leftrightarrow \frac{1}{1-\theta_2} \leq \frac{2}{\phi^2}
\end{align*}
%%
where $\phi$ is the ``conductance'' of $\bm{P}$, which satisfies the following inequality
%%
\begin{align*}
\phi & \geq \min_{\statevec \ne \statevec', P(\statevec, \statevec') > 0} \{  \steadystate_{\rm min}^{\mpliervec(k)} \cdot P(\statevec, \statevec') \} \\
& \geq \steadystate_{\rm min}^{\mpliervec(k)} \cdot Q_{k+1}^{\rm min} / Q_{k+1}^{\rm max}.
\end{align*}
%%
Therefore we obtain
%%
\begin{align}
\label{eqn:proof-slev-bound}
\frac{1}{1-\slev} \leq \frac{2}{\phi^2} \leq 2 \left( \frac{Q_{k+1}^{\rm max}}{ \steadystate_{\rm min}^{\mpliervec(k)} \cdot Q_{k+1}^{\rm min}} \right)^{2}.
\end{align}
%%

Putting everything back into the estimation, we have
%%
\begin{align*}
& \onenorm{ \expectation{ \powerconsemp_i(k+1) | \markovhist_k } - \powercons_i(k+1)} \\
& = \onenorm{ \listencost{i} (\listenfracemp{i}(k+1) - \listenfrac{i}(k+1)) + \xmitcost{i} (\xmitfracemp{i}(k+1) - \xmitfrac{i}(k+1)) } \\
& \leq \listencost{i} \onenorm{ \listenfracemp{i}(k+1) - \listenfrac{i}(k+1) } + \xmitcost{i} \onenorm{ \xmitfracemp{i}(k+1) - \xmitfrac{i}(k+1) }.
% & \leq \costmax \cdot \normtv{ \bar{\mu} - \steadystate(\mpliervec(k))},
\end{align*}
%%
Furthermore, we have
%%
\begin{align*}
& \onenorm{ \listenfracemp{i}(k+1) - \listenfrac{i}(k+1) } \\
& = \onenorm{ \sum\limits_{\statevec \in \statespace_i^l} \int_{t_{k}}^{t_{k+1}} ( \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} ) \, \textrm{d}t / \epoch_{k+1} } \\
% & \leq \sum\limits_{\statevec \in \statespace_i^l} \int_{t_{k}}^{t_{k+1}} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} } \, \textrm{d}t / \epoch_{k+1} \\
& \leq \int_{t_{k}}^{t_{k+1}} \sum\limits_{\statevec \in \statespace_i^l} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} } \, \textrm{d}t / \epoch_{k+1}.
\end{align*}
%%
Similarly,
%%
\begin{align*}
& \onenorm{ \xmitfracemp{i}(k+1) - \xmitfrac{i}(k+1) } \\
& \leq \int_{t_{k}}^{t_{k+1}} \sum\limits_{\statevec \in \statespace_i^x} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} } \, \textrm{d}t / \epoch_{k+1}.
\end{align*}
%%
Adding both terms together we obtain
%%
\begin{align*}
& \listencost{i} \onenorm{ \listenfracemp{i}(k+1) - \listenfrac{i}(k+1) } + \xmitcost{i} \onenorm{ \xmitfracemp{i}(k+1) - \xmitfrac{i}(k+1) } \\
& \leq \costmax \int_{t_k}^{t_{k+1}} \sum_{\statevec \in \statespace} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} } \, \textrm{d}t / \epoch_{k+1} \\
& \leq \frac{\costmax}{\sqrt{\steadystate_{\rm min}^{\mpliervec(k)}}} \int_{t_k}^{t_{k+1}} \exp{(-Q_{k+1}^{\rm max}(1-\slev)t)} \, \textrm{d}t / \epoch_{k+1} ~\textrm{(use~\eqref{eqn:proof-norvtv-bound})} \\
& \leq \frac{\costmax}{\sqrt{\steadystate_{\rm min}^{\mpliervec(k)}}} \int_{0}^{t_{k+1}} \exp{(-Q_{k+1}^{\rm max}(1-\slev)t)} \, \textrm{d}t / \epoch_{k+1} \\
& \leq \frac{\costmax}{\sqrt{\steadystate_{\rm min}^{\mpliervec(k)}}} \cdot \frac{1}{2 Q_{k+1}^{\rm max} (1-\slev)} \cdot \frac{1}{\epoch_{k+1}} \\
& \leq \frac{\costmax Q_{k+1}^{\rm max}}{ (Q_{k+1}^{\rm min})^2 (\steadystate_{\rm min}^{\mpliervec(k)})^{5/2} } \cdot \frac{1}{\epoch_{k+1}} := \frac{f(k)}{\epoch_{k+1}}, ~\textrm{(use~\eqref{eqn:proof-slev-bound})}
\end{align*}
%%
in which
%%
\begin{align*}
f(k) := \frac{\costmax Q_{k+1}^{\rm max}}{ (Q_{k+1}^{\rm min})^2 (\steadystate_{\rm min}^{\mpliervec(k)})^{5/2} }.
\end{align*}
%%
Therefore we have,
%%
\begin{align*}
\onenorm{ \expectation{ \powerconsemp_i(k+1) | \markovhist_k } - \powercons_i(\mpliervec(k)) } \leq f(k) / \epoch_{k+1},
\end{align*}
%%
%%
and the error term, defined in~\eqref{eqn:proof-gradient-err}, satisfies $\onenorm{ \gradient_i^{\rm err}(k+1)} \leq f(k) / \epoch_{k+1}$. Therefore, with defined $f(k)$ and proper choice of $\epoch_{k+1}$ (e.g., $\epoch_{k+1} = k+1$), the error term is diminishing.


% Since $\onenorm{\mplier_i(k) - \mplier_k^*} \leq \max\nolimits_{i} \mplier_i^* + \costmax \sum\nolimits_{m=1}^k \stepsize_{m}$, we can show that the term $(\mpliervec(k) - \mpliervec^*(k))^T \cdot \gradientvec^{\rm err}(k+1)$ is diminishing:
% %%
% \begin{align}
% \label{eqn:proof-gradient-error-bound}
% & \sum\limits_{k=0}^{+\infty} \left( \stepsize_{k+1} \onenorm{ ( \mpliervec(k) - \mpliervec^* )^{T} \cdot \gradientvec^{\rm err}(k+1) } \right) \nonumber \\
% & \leq \numnode \sum\limits_{k=0}^{+\infty} [ \stepsize_{k+1} (\max\limits_{i} \mplier_i^* + \costmax \sum\limits_{m=1}^k \stepsize_{m}) f(k) / \epoch_{k+1} ] \nonumber \\
% % & = \numnode \costmax \cdot \sum\limits_{k=0}^{+\infty} [ \stepsize_{k+1} \cdot ( \sum\limits_{k'=1}^k \stepsize_{k'}) \cdot f(k) / \epoch_{k+1} ] \nonumber \\
% % & \quad~ + \numnode \costmax \cdot \max\limits_{i} \mplier_i^* \cdot \sum\limits_{k=0}^{+\infty} [ \stepsize_{k+1} \cdot f(k) / \epoch_{k+1} ]
% & < +\infty
% \end{align}
% where the last inequality comes from the condition~\eqref{eqn:proof-aux-constraint}.
% %%


%%
\noindent\textbf{Proof of Part 2}.
The main results of this part is summarized in the following lemma, and the proof is similar to the proof of Theorem~1 in\cite{jiang2009convergence}.
%% begin of lemma
\begin{mylemma}
If~\eqref{eqn:proof-stepsize-constraint-2} and~\eqref{eqn:proof-aux-constraint} hold, then with {\name}, $\mpliervec$ converges to $\mpliervec^*$ with probability 1.
\end{mylemma}
%% end of lemma

Combining Part 1 and Part 2, we complete the proof of Theorem~\ref{thm:convergence}.  \hfill $\Box$

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper"
%%% End:


==> tex/proof_theorem.tex <==
\section{Detailed Proof of Theorem 1}
\label{append:proof-convergence}

The proof of Theorem~\ref{thm:convergence} uses similar techniques as in the proof of Theorem 1 in~\cite{jiang2009convergence} with minor modifications.

%% notations of the proof
\subsection{Some Notation}
We use the same notation described in Appendix~\ref{append:proof-dbe}. Moreover, we have the following notation. We let $\numstate = \onenorm{\statespace}$ denote the total number of network states. Recall that each interval $k$ ($k = 1, 2, \cdots$) starts at time $t_{k-1}$ and ends at time $t_k$, and $t_0=0$. The Lagrangian multiplier $\mpliervec(k)$ is updated at the end of the $k$-th interval. The $k$-th interval is of the length $\epoch_{k} = t_{k} - t_{k-1}$. At time $t$, the probability of the system being in state $\statevec$ is denoted by $\networkprob_{\statevec}(t)$. Notice that throughout the $k$-th interval, $\mpliervec(k-1)$ remains changed and is updated at each node $i$ at time $t_{k}$ according to
%%
\begin{align}
\label{eqn:proof-update-lm-emp}
\mplier_{i}(k) = [ \mplier_{i}(k-1) - \stepsize_{k} ( \powerharv_{i} - \powerconsemp_{i}(k) ) ]^+,
\end{align}
%%
in which $\powerconsemp_i(k)$ is the \textit{empirical} energy consumption rate of node $i$ in the $k$-th interval.\footnote{Although we assume a constant power budget of $\powerharv_i$ at each node $i$, the proof can be easily extended to scenarios where $\powerharv_i$ varies with time.} The empirical energy consumption rate is given by
%%
\begin{align*}
\powerconsemp_i(k) & = \int_{t_{k-1}}^{t_{k}} ( \listencost{i} \prob \left\{ \state_i(t) = l \right\} + \xmitcost{i} \prob \left\{ \state_i(t) = x \right\} )\, \textrm{d}t / \epoch_{k}, \\
& := \listencost{i} \cdot \listenfracemp{i}(k) + \xmitcost{i} \cdot \xmitfracemp{i}(k),
% & = \frac{1}{\epoch_{k}} \int_{t_{k-1}}^{t_{k}} [ \listencost{i} \cdot \nu_{\state_i=l}(t) + \xmitcost{i} \cdot \nu_{\state_i=x}(t) ]\, \textrm{d}t,
\end{align*}
%%
in which $\listenfracemp{i}(k)$ and $\xmitfracemp{i}(k)$ are the empirical fractions of time node $i$ spend in listen and transmit states, in the $k$-th interval. The relationship between the empirical energy consumption rate and the energy storage levels (or battery values) of node $i$, $\bat_i(t)$, is given by $\powerharv_{i} - \powerconsemp_{i}(k) = [ \bat_{i}(t_{k}) - \bat_{i}(t_{k-1}) ] / \epoch_{k}$,
which can be simply obtained from reading the energy storage levels.

In addition, let $\statevec^0(k)$ denote the state of the network Markov chain at the beginning of the $k$-th interval (i.e., at time $t_{k-1}$). Define the random vector $\mathbf{U}(k-1) := [ \powerconsempvec(k-1), \mpliervec(k-1), \statevec^0(k-1) ]$. For $k \geq 1$, let $\markovhist_{k-1}$ be the $\sigma$-field generated by $\mathbf{U}(0), \mathbf{U}(1), \cdots, \mathbf{U}(k-1)$.

In the $k$-th interval, define the gradient vector as $\gradientvec(k) = [\gradient_i(k)]$ whose $i$-th element $\gradient_i(k) = \powerharv_i(k) - \powercons_i(k)$. Given vector $\mpliervec(k-1)$, $\gradientvec(k)$ is a gradient of $\mathcal{L}(\mpliervec)$ (recall that the dual problem of {\namecp} is $\min\nolimits_{\mpliervec \succeq \bm{0}} \mathcal{L}(\mpliervec)$). To find the optimal $\mpliervec^*$ that solves the dual problem, the ideal algorithm (i.e., Algorithm~\ref{alg:gradient-descent}) uses the accurate descent direction of the gradient $\gradientvec$. However, {\name} follows~\eqref{eqn:proof-update-lm-emp} and only has an empirical estimation of $\gradientvec(k)$, denoted by $\gradientempvec(k) = [\gradientemp_i(k)]$, in which $\gradientemp_i(k) = \powerharv_i - \powerconsemp_i(k)$. The ``error'' term is given by $\gradientvec^{\rm err}(k) = [\gradient_i^{\rm err}(k)]$ in which
%%
\begin{align}
\label{eqn:proof-gradient-err}
\gradient_i^{\rm err}(k) & = \expectation{\gradientemp_i(k) | \markovhist_{k-1}} - \gradient_i(k) \nonumber \\
& = \powercons_i(k) - \expectation{ \powerconsemp_i(k) | \markovhist_{k-1} },
\end{align}
%%
The ``noise'' term is given by $\gradientvec^{\rm noise}(k) = [\gradient_i^{\rm noise}(k)]$ with
%%
\begin{align}
\label{eqn:proof-gradient-noise}
& \gradient_i^{\rm noise}(k) = \expectation{ \powerconsemp_i(k) | \markovhist_{k-1} } -  \powerconsemp_i(k).
\end{align}
%%
Therefore we can write the empirical gradient as
%%
\begin{align*}
\gradientemp_i(k) = \gradient_i(k) + \gradient_i^{\rm err}(k) + \gradient_i^{\rm noise}(k), ~\forall i \in \setnodes.
\end{align*}
%%
Notice that since $\powerharv_i(k)$ and $\powerconsemp_i(k)$ are both bounded, therefore the noise term is also bounded by some constant, i.e.,
%%
\begin{align*}
\onenorm{\gradient_i^{\rm noise}(k)} \leq \gradientmax^{\rm noise}, ~\forall i \in \setnode.
\end{align*}
%%

\subsection{Proof of Convergence}
% summary of proof
The proof is composed of two parts. In part 1, we show that with {\name}, the error term $\gradientvec^{\rm err}(k)$~\eqref{eqn:proof-gradient-err} decreases ``fast enough'' with time. In part 2, we show that $\mpliervec$ converge to $\mpliervec^*$ with probability $1$ (w.p.$1$). We provide the detailed proof or part 1 below and the proof of part 2 is similar to the proof or Theorem 1 in~\cite{jiang2009convergence}.

%%
We assume that the step size $\stepsize_{k} > 0$ and the following conditions hold.
%%
\begin{align}
\label{eqn:proof-stepsize-constraint}
& \sum\limits_{k=0}^{+\infty} \stepsize_{k} = +\infty, ~\sum\limits_{k=0}^{+\infty} \stepsize_{k}^{2} < +\infty \\
\label{eqn:proof-stepsize-constraint-2}
& \sum\limits_{k=0}^{+\infty} \left( \stepsize_{k+1} \sum\limits_{m=1}^{k} \stepsize_{m} \right)^2 < +\infty, \\
\label{eqn:proof-aux-constraint} % auxiliary constraint
& \sum\limits_{k=0}^{+\infty} \left[ \stepsize_{k+1} (\max\limits_{i} \mplier_{i}^{*} + \costmax 
\sum\limits_{m=1}^{k} \stepsize_{m}) f(k) / \epoch_{k+1} \right] < +\infty,
\end{align}
%%
in which, 
%%
\begin{align*}
& \costmax = \max\limits_{i} \{ \max \{ \listencost{i}, \xmitcost{i} \} \}, \quad \xi_k = \costmax^{2} \sum\limits_{m=1}^{k} \stepsize_{m}, \\
& f(k) = 2\numnode \costmax \numstate^{5/2} \cdot \exp ( 3\xi_{k} + \frac{5}{2} \numnode (\xi_k+1) ).
\end{align*}
%%
It can be easily verified that $\stepsize_{k} = 1/[(k+1)\log{(k+1)}]$ and $\epoch_{k} = k$ satisfy all the above conditions.


%%%%% BEGIN OF PROOF OF CONVERGENCE %%%%%

% proof of part 1: error term is decreasing fast enough
\noindent\textbf{Proof of Part 1}.
We drop the index $(k+1)$ and denote the Continuous-Time Markov chain (CTMC) in the $(k+1)$-th interval by $X(t),~\forall t \in [t_k, t_{k+1})$. For brevity, we assume $\oursigma=1$ and drop the term $1/\oursigma$. From~\eqref{eqn:steady-state-prob}, the {\em steady state distribution} of $X(t)$ with given $\mpliervec(k)$ is given by
%%
\begin{align*}
\steadystate_{\statevec}^{\mpliervec(k)} = \exp [ \tput_{\statevec} - \sum\limits_{i \in \setnode_l(\statevec)} \mplier_i(k) \listencost{i} - \sum\limits_{i \in \setnode_x(\statevec)} \mplier_i(k) \xmitcost{i} ] / Z^{\mpliervec(k)}
\end{align*}
%%
where $Z^{\mpliervec(k)}$ is a constant such that $\sum_{\statevec \in \statespace} \steadystate_{\statevec}^{\mpliervec(k)} = 1$. This constant can be bounded by
%%
\begin{align*}
& \sum_{\statevec \in \statespace} \exp \left[ \tput_{\statevec} - \sum_{i \in \setnode_l(\statevec)} \mplier_i(k) \listencost{i} - \sum_{i \in \setnode_x(\statevec)} \mplier_i(k) \xmitcost{i} \right] \\
& \quad \leq \numstate \cdot \exp{(\numnode)} = (2+\numnode) \cdot 2^{\numnode-1} \cdot \exp(\numnode),
\end{align*}
%%
in which the inequality comes from the fact that $\tput_{\statevec} \leq \numnode$. On the other hand, we also have
%%
\begin{align*}
& \exp \left[ \tput_{\statevec} - \sum\limits_{i \in \setnode_l(\statevec)} \mplier_i(k) \listencost{i} - \sum\limits_{i \in \setnode_x(\statevec)} \mplier_i(k) \xmitcost{i} \right] \\
& \quad \geq \exp [ - \numnode \cdot \costmax \cdot \max\limits_i \{ \mplier_i(k) \} ]
\end{align*}
%%
where $\costmax := \max\nolimits_{i \in \setnodes} \left\{ \max \left\{ \listencost{i}, \xmitcost{i} \right\} \right\}$. According to the updates of $\mpliervec(k)$, $\max\nolimits_i \{ \mplier_i(k) \}$ can be further bounded by $\max\nolimits_{i \in \setnodes} \{\mplier_{i}(k)\} \leq \costmax \cdot \sum\nolimits_{m=1}^{k} \stepsize_{m}$. Therefore, denoting $\xi_{k} := \costmax^{2} \cdot \sum\nolimits_{m=1}^{k} \stepsize_{m}$, we have the minimum probability in the stationary distribution lower bounded by
%%
\begin{align}
\label{eqn:proof-steadystate-min}
\steadystate_{\statevec}^{\mpliervec(k)} \geq \frac{\exp ( - \xi_{k} \numnode )}{ \numstate \cdot \exp(\numnode)} := \steadystate_{\rm min}^{\mpliervec(k)}.
\end{align}
%%

Before proceeding with the proof, we first state the following useful propositions.

%% begin of prop
\begin{proposition}
Denote $\bm{Q} = [Q(\statevec, \statevec')]$ as the transition rate matrix of $X(t)$ in the $(k+1)$-th interval. If $Q(\statevec, \statevec') > 0$, there exists $Q_{\rm max} \geq Q_{\rm min} > 0$ such that
%%
\begin{align*}
Q_{k+1}^{\rm min} \leq Q(\statevec, \statevec') \leq Q_{k+1}^{\rm max}.
\end{align*}
%%
%In particular, $Q_{k+1}^{\rm max} := 2\numnode \exp(\xi_{k})$ and $Q_{k+1}^{\rm min} = \exp{(-\xi_{k})}$ are suffice.
%Furthermore, there is at most $2\numnode$ states $\statevec' \ne \statevec$ that can have positive transition rates $Q(\statevec, \statevec') > 0$.
\end{proposition}
%% end of prop
%% begin of proof
\begin{IEEEproof}
Given state $\statevec = [\state_i]$, there is a total number of $\numnode_s(\statevec) + 2\numnode_l(\statevec) + \numnode_x(\statevec) \leq 2\numnode$ states $\statevec'$ other than $\statevec$ that $X(t)$ can transition to. Recall that for any state $\statevec' \ne \statevec$, we have for each node $i$,
%%
\begin{align}
\label{eqn:trans-rate-matrix}
& Q(\statevec, \statevec') \nonumber \\
& = \left\{
\begin{aligned}
& \exp [ - \mplier_i(k) \listencost{i} ], && \state_i=s \to \state_i=l \\
& \exp [ \mplier_i(k) (\listencost{i} - \xmitcost{i}) ], && \state_i=l \to \state_i=x \\
& 1, && \state_i=l \to \state_i=s \\
& \exp( - \tput_{\statevec}),. && \state_i=x \to \state_i=l
\end{aligned}
\right.
\end{align}
%%
It is easy to see that the transition rate is always bounded, and $Q_{k+1}^{\rm min} = \min\{ \exp(-\numnode), \exp(-\xi_k) \}$ will suffice. In particular, given the network size $\numnode$, for sufficiently large $k$, $\xi_k > \numnode$ holds, and therefore we use $Q_{k+1}^{\rm min} := \exp(-\xi_{k})$.

On the other hand, if for $\listencost{i} \leq \xmitcost{i}, \forall i \in \setnodes$, each one of the $2\numnode$ transition rates in~\eqref{eqn:trans-rate-matrix} is less than or equal to $1$, and $Q_{k+1}^{\rm max} = 2\numnode$ is sufficient. Second, if there exists some node $i$ such that $\listencost{i} > \xmitcost{i}$, beacause of the costs are always upper bounded by $\costmax$, the transition rate is also upper bounded by $\exp(\costmax \mpliermax) \leq \exp{(\costmax^{2} \sum\nolimits_{m=1}^{k} \stepsize_{m})} = \exp{(\xi_{k})}$. Therefore $Q_{k+1}^{\rm max} = 2\numnode \exp{(\xi_{k})}$ is sufficient.
\end{IEEEproof}
%% end of proof

Following the regular process, we first perform uniformization of the continuous time Markov chain $X(t)$. For the Markov chian $X(t)$, if each element of its transition rate matrix $\bm{Q}$ has an absolulte value less that a constant $Q_{k+1}^{\rm max}$, then we can write $X(t) = Y(M(t))$, in which $Y(n)$ is a discrete time Markov chain with probability transition matrix $\bm{P} = \bm{I} + \bm{Q} / Q_{k+1}^{\rm max}$ and $\bm{I}$ is the identity matrix. $M(t)$ is an independent Poisson process with rate $Q_{k+1}^{\rm max}$.
% Recall that $Q(\statevec, \statevec') > 0$ for {\it at most} $2\numnode$ different states $\statevec' \ne \statevec$. We have the following proposition which gives a value of $A_{k+1}$ that is sufficient for the uniformization.

% %% begin of prop
% \begin{proposition}
% The following value of $A_{k+1}$ is sufficient for the uniformization,
% %%
% \begin{align}
% \label{eqn:proof-uniformization-rate}
% A_{k+1} := 2\numnode \exp(\xi_{k}),
% \end{align}
% %%
% \end{proposition}
% %% end of prop
% %% proof of prop
% \begin{proof}
% First, if for $\listencost{i} \leq \xmitcost{i}, \forall i \in \setnodes$, each one of the $2\numnode$ transition rates in~\eqref{eqn:trans-rate-matrix} is less than or equal to $1$, and $A_{k+1} = 2\numnode$ is sufficient. Second, if there exists some node $i$ such that $\listencost{i} > \xmitcost{i}$, beacause of the costs are always upper bounded by $\costmax$, the transition rate is also upper bounded by $\exp(\costmax \mpliermax) \leq \exp{(\costmax^{2} \sum\nolimits_{m=1}^{k} \stepsize_{m})} = \exp{(\xi_{k})}$. Thus $A_{k+1} = 2\numnode \exp{(\xi_{k})}$ is sufficient. Since $\xi_{k} \geq 0$ holds, using $A_{k+1}$ defined as in (\ref{eqn:proof-uniformization-rate}), the uniformization is valid.
% \end{proof}
% %% end of proof

We estimate how far the empirical power consumption $\expectation{\powerconsemp_i(k+1) | \markovhist_k}$ is away from the desired value $\powercons_{i}(k+1)$ (under fixed $\mpliervec(k)$). Denote the probability of $X(t)$ in state $\statevec$ at time $t \in [t_{k}, t_{k+1})$ by $\networkprob_{\statevec}(t)$ and $\networkprobvec(t) = [\networkprob_{\statevec}(t)]$. Given the initial state at time $t_k$ is $\statevec^0(k+1)$, We have
%%
\begin{align*}
& \expectation{ \powerconsemp_i(k+1) | \markovhist_k }\\
& = \expectation{ \int_{t_k}^{t_{k+1}} \sum_{\statevec \in \statespace} \left( \mathbf{1}_{ 
\{\state_i = l\} } \listencost{i} +  \mathbf{1}_{ \{ \state_i = x \} } \xmitcost{i} \right)\, \textrm{d}t / \epoch_{k+1} } \\
& = \int_{t_k}^{t_{k+1}} \sum_{\statevec \in \statespace} ( \prob \left\{ \state_i(t) = l \right\} \listencost{i} + \prob \left\{ \state_i(t) = x \right\} \xmitcost{i} )\, \textrm{d}t / \epoch_{k+1} \\
& = \frac{\listencost{i}}{\epoch_{k+1}} \sum_{\statevec \in \statespace_i^l} \int_{t_k}^{t_{k+1}} \networkprob_{\statevec}(t)\, \textrm{d}t + \frac{\xmitcost{i}}{\epoch_{k+1}} \sum_{\statevec \in \statespace_i^x} \int_{t_{k}}^{t_{k+1}} \networkprob_{\statevec}(t)\, \textrm{d}t \\
& = \listencost{i} \cdot \listenfracemp{i}(k+1) + \xmitcost{i} \cdot \xmitfracemp{i}(k+1),
\end{align*}
%%
in which
%%
\begin{align*}
& \emplistenfrac{i}(k+1) = \sum\limits_{\statevec \in \statespace_i^l} \int_{t_{k}}^{t_{k+1}} \networkprob_{\statevec}(t) \, \textrm{d}t / \epoch_{k+1} \\
& \xmitfracemp{i}(k+1) = \sum\limits_{\statevec \in \statespace_i^x} \int_{t_{k}}^{t_{k+1}} \networkprob_{\statevec}(t) \, \textrm{d}t / \epoch_{k+1}
\end{align*}
%%
are the empirical average probabilities that node $i$ spends in listen and transmit states in the $(k+1)$-th interval.

Let $\slev$ with $|\slev| \leq 1$ be the Second Largest Eigenvalue of the transition probability matrix $\bm{P} = \bm{I} + \bm{Q} / Q_{k+1}^{\rm max}$, and define the total variation distance by $\norm{\cdot}_{\rm TV}$, i.e.,
%%
\begin{align*}
\normtv{\networkprobvec(t) - \steadystatevec^{\mpliervec(k)}} = \frac{1}{2} \sum\limits_{\statevec \in \statespace} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} }.
\end{align*}
%%
This total variation distance can be bounded by
%%
\begin{align}
\label{eqn:proof-norvtv-bound}  % total variance bound
\normtv{\networkprobvec(t) - \steadystatevec^{\mpliervec(k)}}
& \leq \frac{1}{2} \sqrt{ \frac{1 - \steadystate_{\statevec^{0}}^{\mpliervec(k)}}{\steadystate_{\statevec^{0}}^{\mpliervec(k)}} } \exp ( - Q_{k+1}^{\rm max} (1-\slev) t) \nonumber \\
& \leq \frac{1}{2} \frac{1}{\sqrt{\steadystate_{\rm min}^{\mpliervec(k)}}} \exp ( - Q_{k+1}^{\rm max} (1-\slev) t). 
\end{align}
%%
Also, the Second Largest Eigenvalue, $\slev$, can be bounded by Cheeger's inequality~\cite{diaconis1991geometric}, i.e.,
%%
\begin{align*}
\slev \leq 1 - \frac{\phi^2}{2} \Leftrightarrow \frac{1}{1-\theta_2} \leq \frac{2}{\phi^2}
\end{align*}
%%
where $\phi$ is the ``conductance'' of $\bm{P}$, which satisfies the following inequality
%%
\begin{align*}
\phi & \geq \min_{\statevec \ne \statevec', P(\statevec, \statevec') > 0} \{  \steadystate_{\rm min}^{\mpliervec(k)} \cdot P(\statevec, \statevec') \} \\
& \geq \steadystate_{\rm min}^{\mpliervec(k)} \cdot Q_{k+1}^{\rm min} / Q_{k+1}^{\rm max}.
\end{align*}
%%
Therefore we obtain
%%
\begin{align}
\label{eqn:proof-slev-bound}
\frac{1}{1-\slev} \leq \frac{2}{\phi^2} \leq 2 \left( \frac{Q_{k+1}^{\rm max}}{ \steadystate_{\rm min}^{\mpliervec(k)} \cdot Q_{k+1}^{\rm min}} \right)^{2}.
\end{align}
%%

Putting everything back into the estimation, we have
%%
\begin{align*}
& \onenorm{ \expectation{ \powerconsemp_i(k+1) | \markovhist_k } - \powercons_i(k+1)} \\
& = \onenorm{ \listencost{i} (\listenfracemp{i}(k+1) - \listenfrac{i}(k+1)) + \xmitcost{i} (\xmitfracemp{i}(k+1) - \xmitfrac{i}(k+1)) } \\
& \leq \listencost{i} \onenorm{ \listenfracemp{i}(k+1) - \listenfrac{i}(k+1) } + \xmitcost{i} \onenorm{ \xmitfracemp{i}(k+1) - \xmitfrac{i}(k+1) }.
% & \leq \costmax \cdot \normtv{ \bar{\mu} - \steadystate(\mpliervec(k))},
\end{align*}
%%
Furthermore, we have
%%
\begin{align*}
& \onenorm{ \listenfracemp{i}(k+1) - \listenfrac{i}(k+1) } \\
& = \onenorm{ \sum\limits_{\statevec \in \statespace_i^l} \int_{t_{k}}^{t_{k+1}} ( \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} ) \, \textrm{d}t / \epoch_{k+1} } \\
% & \leq \sum\limits_{\statevec \in \statespace_i^l} \int_{t_{k}}^{t_{k+1}} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} } \, \textrm{d}t / \epoch_{k+1} \\
& \leq \int_{t_{k}}^{t_{k+1}} \sum\limits_{\statevec \in \statespace_i^l} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} } \, \textrm{d}t / \epoch_{k+1}.
\end{align*}
%%
Similarly,
%%
\begin{align*}
& \onenorm{ \xmitfracemp{i}(k+1) - \xmitfrac{i}(k+1) } \\
& \leq \int_{t_{k}}^{t_{k+1}} \sum\limits_{\statevec \in \statespace_i^x} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} } \, \textrm{d}t / \epoch_{k+1}.
\end{align*}
%%
Adding both terms together we obtain
%%
\begin{align*}
& \listencost{i} \onenorm{ \listenfracemp{i}(k+1) - \listenfrac{i}(k+1) } + \xmitcost{i} \onenorm{ \xmitfracemp{i}(k+1) - \xmitfrac{i}(k+1) } \\
& \leq \costmax \int_{t_k}^{t_{k+1}} \sum_{\statevec \in \statespace} \onenorm{ \networkprob_{\statevec}(t) - \steadystate_{\statevec}^{\mpliervec(k)} } \, \textrm{d}t / \epoch_{k+1} \\
& \leq \frac{\costmax}{\sqrt{\steadystate_{\rm min}^{\mpliervec(k)}}} \int_{t_k}^{t_{k+1}} \exp{(-Q_{k+1}^{\rm max}(1-\slev)t)} \, \textrm{d}t / \epoch_{k+1} ~\textrm{(use~\eqref{eqn:proof-norvtv-bound})} \\
& \leq \frac{\costmax}{\sqrt{\steadystate_{\rm min}^{\mpliervec(k)}}} \int_{0}^{t_{k+1}} \exp{(-Q_{k+1}^{\rm max}(1-\slev)t)} \, \textrm{d}t / \epoch_{k+1} \\
& \leq \frac{\costmax}{\sqrt{\steadystate_{\rm min}^{\mpliervec(k)}}} \cdot \frac{1}{2 Q_{k+1}^{\rm max} (1-\slev)} \cdot \frac{1}{\epoch_{k+1}} \\
& \leq \frac{\costmax Q_{k+1}^{\rm max}}{ (Q_{k+1}^{\rm min})^2 (\steadystate_{\rm min}^{\mpliervec(k)})^{5/2} } \cdot \frac{1}{\epoch_{k+1}} := \frac{f(k)}{\epoch_{k+1}}, ~\textrm{(use~\eqref{eqn:proof-slev-bound})}
\end{align*}
%%
in which
%%
\begin{align*}
f(k) := \frac{\costmax Q_{k+1}^{\rm max}}{ (Q_{k+1}^{\rm min})^2 (\steadystate_{\rm min}^{\mpliervec(k)})^{5/2} }.
\end{align*}
%%
Therefore we have,
%%
\begin{align*}
\onenorm{ \expectation{ \powerconsemp_i(k+1) | \markovhist_k } - \powercons_i(\mpliervec(k)) } \leq f(k) / \epoch_{k+1},
\end{align*}
%%
%%
and the error term, defined in~\eqref{eqn:proof-gradient-err}, satisfies $\onenorm{ \gradient_i^{\rm err}(k+1)} \leq f(k) / \epoch_{k+1}$. Therefore, with defined $f(k)$ and proper choice of $\epoch_{k+1}$ (e.g., $\epoch_{k+1} = k+1$), the error term is diminishing.


% Since $\onenorm{\mplier_i(k) - \mplier_k^*} \leq \max\nolimits_{i} \mplier_i^* + \costmax \sum\nolimits_{m=1}^k \stepsize_{m}$, we can show that the term $(\mpliervec(k) - \mpliervec^*(k))^T \cdot \gradientvec^{\rm err}(k+1)$ is diminishing:
% %%
% \begin{align}
% \label{eqn:proof-gradient-error-bound}
% & \sum\limits_{k=0}^{+\infty} \left( \stepsize_{k+1} \onenorm{ ( \mpliervec(k) - \mpliervec^* )^{T} \cdot \gradientvec^{\rm err}(k+1) } \right) \nonumber \\
% & \leq \numnode \sum\limits_{k=0}^{+\infty} [ \stepsize_{k+1} (\max\limits_{i} \mplier_i^* + \costmax \sum\limits_{m=1}^k \stepsize_{m}) f(k) / \epoch_{k+1} ] \nonumber \\
% % & = \numnode \costmax \cdot \sum\limits_{k=0}^{+\infty} [ \stepsize_{k+1} \cdot ( \sum\limits_{k'=1}^k \stepsize_{k'}) \cdot f(k) / \epoch_{k+1} ] \nonumber \\
% % & \quad~ + \numnode \costmax \cdot \max\limits_{i} \mplier_i^* \cdot \sum\limits_{k=0}^{+\infty} [ \stepsize_{k+1} \cdot f(k) / \epoch_{k+1} ]
% & < +\infty
% \end{align}
% where the last inequality comes from the condition~\eqref{eqn:proof-aux-constraint}.
% %%


%%
\noindent\textbf{Proof of Part 2}.
The main results of this part is summarized in the following lemma, and the proof is similar to the proof of Theorem~1 in\cite{jiang2009convergence}.
%% begin of lemma
\begin{mylemma}
If~\eqref{eqn:proof-stepsize-constraint-2} and~\eqref{eqn:proof-aux-constraint} hold, then with {\name}, $\mpliervec$ converges to $\mpliervec^*$ with probability 1.
\end{mylemma}
%% end of lemma

Combining Part 1 and Part 2, we complete the proof of Theorem~\ref{thm:convergence}.  \hfill $\Box$

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../conext16"
%%% End:


==> tex/simulation_conext.tex <==
\section{Numerical Results}
\label{sec:sim}

%% what we do 
In this section, we consider various heterogeneous networks and numerically show that the throughput approaches the oracle throughput $\UB$ as $\oursigma$ decreases. In the special case of homogeneous networks, we explore the sensitivity of the throughput to various power consumption levels, and compare to related work. Then, via simulations, we study the burstiness and latency of {\name}, and evaluate its performance in non-clique topologies.

% Our general conclusions with respect to anyput performance are quite similar as to groupput. Therefore, we focus on the \textit{groupput performance achieved by {\namecap}} throughout this section.
For brevity, we omit the subscript for groupput and use the following notation: (i) $\UB$ is the oracle groupput obtained by solving {\namelp} or, equivalently, {\namelpgput}, (ii) $\gputsigma$ is the achievable groupput of {\name} with a given value of $\oursigma$ obtained by solving {\namecp}, and (iii) $\gputsigmasim$ is the groupput of {\name} obtained via simulations with a given value of $\oursigma$.

%% evaluation setup
\subsection{Setup}
\label{ssec:sim-setup}
We consider $\oursigma \in \{0.1, 0.25, 0.5\}$. The nodes' power budgets and consumption levels correspond to energy harvesting budgets and ultra-low-power transceivers in~\cite{Gorlatova_NetworkingLowPower, gorlatova2015movers, philips2014ultra}. Unless stated otherwise, we use a power budget of $\energybound{} = \ouruW{10}$ and power consumption levels $\listencost{} = \xmitcost{} = \ourmW{0.5}$. This results in a ratio of $50$ between the transceiver power consumption and the budget. Note that the performance of {\name} only depends on the \textit{ratio} between the listen or transmit power and the power budget. For example, nodes with $\energybound{} = \ouruW{10}, \listencost{} = \xmitcost{} = \ourmW{0.5}$ behave exactly the same as nodes with $\energybound{} = \ourmW{1}, \listencost{} = \xmitcost{} = \ourmW{50}$. Therefore, the oracle throughput applies and {\name} can operate in very general settings.

Recall that we assume that there are not simultaneous transmissions and collisions. We also assume that the packet length is $\ourms{1}$ and that nodes have accurate estimate of the number of listeners, i.e., $\numlistenest(t) = \numlisten(t)$. 

Our simulation results show that $\gputsigmasim$ perfectly matches $\gputsigma$ for $\oursigma \in \{0.25, 0.5\}$. For $\oursigma = 0.1$, $\gputsigmasim$ does not converge to $\gputsigma$ within reasonable time due to the bursty nature of {\name}, as will be described in Section~\ref{ssec:sim-burstiness}. Therefore, we evaluate the throughput performance of {\name} by comparing $\gputsigma$ to $\UB$ with varying $\oursigma$ in both heterogeneous and homogeneous networks. Specifically, \textit{homogeneous networks} consist of nodes with the same power budget and consumption levels, i.e., $\energybound{i} = \energybound{}, \listencost{i} = \listencost{}, \xmitcost{i} = \xmitcost{},\forall i \in \setnodes$.


%%
% - hetnet evaluation
\subsection{Heterogeneous Networks -- Throughput}
\label{ssec:sim-het-net}

%% only gput
% generated using plot_tput_hetnet.m
% path: ./fig/analysis_figs/
% \begin{figure}[!t]
% \begin{center}
% \includegraphics[width=0.80\columnwidth]{figs/analysis_figs/analysis_hetnet.pdf}
% \caption{Sensitivity of the achievable throughput normalized to the oracle throughput, $\gputsigma/\UB$, to the heterogeneity of the power budget, $\energybound{}$, and consumption levels, $\listencost{}$ and $\xmitcost{}$.}
% \label{fig:analysis-hetnet}
% \vspace{-1.5\baselineskip}
% \end{center}
% \end{figure}
%%

%% gput and aput
\begin{figure}[!t]
\centering
\vspace{-0.75\baselineskip}
\subfloat[]{
\label{fig:sim-hetnet-gput}
\includegraphics[width=0.48\columnwidth]{figs/analysis_figs/hetnet_gput.eps}
}
\hspace{-18pt} \hfill
\subfloat[]{
\label{fig:sim-hetnet-aput}
\includegraphics[width=0.48\columnwidth]{figs/analysis_figs/hetnet_aput.eps}
}
\vspace{-0.5\baselineskip}
\caption{Sensitivity of the achievable throughput normalized to the oracle throughput, $\tputsigma/\UB$, for: (a) groupput and (b) anyput, to the heterogeneity of the power budget, $\energybound{}$, and power consumption levels, $\listencost{}$ and $\xmitcost{}$.}
\label{fig:sim-hetnet}
\vspace{-\baselineskip}
\end{figure}
%%

One strength of {\name} is its ability to deal with \textit{heterogeneous} networks. Figure~\ref{fig:analysis-hetnet} shows the throughput achieved by {\name} normalized to the corresponding oracle throughput (i.e., $\gputsigma/\UB$) for heterogeneous networks with $\numnode = 5$ and $\oursigma \in \{0.1, 0.25, 0.5\}$. The results are obtained by solving {\namelp} for $\UB$ and {\namecp} for $\gputsigma$ with a given value of $\oursigma$. Intuitively, higher values of $\gputsigma/\UB$ indicate better performance of {\name}.

Along the $x$-axis, the \textit{network heterogeneity}, denoted by $h$, is varied from $10$ to $250$ at discrete points. The relationship between the network heterogeneity and the values of $h$ is as follows: (i) for each node $i$, $\listencost{i}$ and $\xmitcost{i}$ are independently selected from a uniform distribution on the interval $[510-h, 490+h]~(\ouruW{})$, (ii) for each node $i$, a variable $h'$ is first sampled from the interval $[-\log{\frac{h}{100}}, \log{h}]$ uniformly at random, and then $\energybound{i}$ is set to be $\exp{(h')}$. Therefore, the energy budget $\energybound{i}$ varies from $100/h$ to $h~(\ouruW{})$. As a result, for any $h$, $\listencost{i}$ and $\xmitcost{i}$ have mean values of $\ourmW{0.5}$. $\energybound{i}$ has median of $\ouruW{10}$ but its mean increases as $h$ increases. Note that a homogeneous network is represented by $h=10$.

The $y$-axis indicates for each value of $h$, the mean and the $95\%$ confidence interval of the ratios $\gputsigma/\UB$ averaged over $1000$ heterogeneous network samples. Figure~\ref{fig:analysis-hetnet} shows that $\gputsigma/\UB$ approaches $1$ as $\oursigma$ decreases, illustrating the results in Section~\ref{sec:algorithm}. Furthermore, with increased heterogeneity of the network, $\gputsigma/\UB$ has little dependency on the heterogeneity but heavy dependency on $\oursigma$. Since larger $h$ values impose higher power budgets, the corresponding oracle throughput $\UB$ increases as well.


%%
% - homogeneous network
% - comparison to related work
\subsection{Homogeneous Networks -- Comparison to Related Work }
\label{ssec:sim-tput}
We now evaluate the performance of {\name} in \textit{homogeneous} networks with repest to different power consumption levels, and compare to related work which assumes homogeneity across nodes. We consider three protocols: \textit{Panda}~\cite{PANDA}, \textit{Birthday}~\cite{McGlynn_mobihoc01}, and \textit{Searchlight}~\cite{Bakht_mobicom2012}, which operate under stricter assumptions than {\name}. In particular:
\begin{itemize}
\item
The probabilistic protocols Panda and Birthday both require a homogeneous set of nodes and a priori knowledge of the number of nodes, $\numnode$. The throughput of Panda and Birthday is computed as described in~\cite{PANDA} and~\cite{McGlynn_mobihoc01}, respectively.
\item
The deterministic protocol Searchlight is designed for minimizing the worst case pairwise discovery latency, which does not directly address multi-party communication across a shared medium. However, the discovery latency is closely related to the throughput, since the inverse of the average latency is the throughput. Hence, maximizing throughput is equivalent to minimizing the average discovery latency. We derive an upper bound on the throughput of Searchlight by multiplying the pairwise throughput by $(\numnode-1)$. This is assuming that all other $(\numnode-1)$ nodes will be receiving when one node transmits. However, in practice the throughput is likely to be lower unless all the nodes are synchronized and coordinated.
\end{itemize}

%%
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.8\columnwidth]{figs/analysis_figs/analysis_tput.pdf}
\caption{Throughput performance of various protocols (all normalized to the oracle throughput $\UB$) with $\numnode = 5$, $\energybound{} = \ouruW{10}$, and $\listencost{} + \xmitcost{} = \ourmW{1}$, as a function of $\xmitcost{} / \listencost{}$.
}
\label{fig:analysis-compare-bounds-groupput}
\vspace{-1.5\baselineskip}
\end{center}
\end{figure}
%%
Figure~\ref{fig:analysis-compare-bounds-groupput} presents the throughput achieved by various protocols normalized to the oracle throughput $\UB$ as a function of the ratio $\xmitcost{} / \listencost{}$, with $\numnode = 5$, $\energybound{} = \ouruW{10}$, and $\listencost{} + \xmitcost{} = \ourmW{1}$. The protocols considered are: {\name} with $\oursigma \in \{0.1, 0.25, 0.5\}$, Panda, Birthday, and Searchlight.\footnote{For Searchlight we compare its throughput upper bound to $\UB$, as described in Section~\ref{ssec:sim-tput}.} The horizontal dashed line at $1$ represents the oracle throughput. Note that with $\listencost{} = \xmitcost{} = \ourmW{0.5}$, the ratio $\gputsigma/\UB$ achieved by {\name} outperforms that of Panda by $6$x and $17$x with $\oursigma = 0.5$ and $\oursigma = 0.25$, respectively. The simulation results, which will be discussed later, also verify this throughput improvement.

Figure~\ref{fig:analysis-compare-bounds-groupput} shows that with $\oursigma=0.1$, $\gputsigma$ is very close to the oracle throughput $\UB$ unless $\xmitcost{} \ll \listencost{}$. As $\oursigma$ is increased, the ratio $\gputsigma/\UB$ drops as expected (see Section~\ref{sec:algorithm}) but still significantly outperforms that of prior art for $\xmitcost{} \approx \listencost{}$. However, the performance of {\name} degrades with extreme values of $\xmitcost{}/\listencost{}$. This is because with small $\xmitcost{}/\listencost{}$ values, nodes enter transmit state infrequently, since listen is expensive and they must pass the listen state to enter the transmit state. On the other hand, with large $\xmitcost{}/\listencost{}$ values, nodes waste their energy to transmit even when there is no other nodes listening (e.g., $\numlistenest(t)=0$). We believe that any distributed protocol will suffer from such performance degradation since, unlike Panda, Birthday, and Searchlight, nodes in a fully distributed setting \textit{do not} have any information about the properties of other nodes in the network.


%%
% - burstiness
% - delay tolerance
\subsection{Burstiness and Latency}
\label{ssec:sim-burstiness}

The results until now suggest allowing $\oursigma \to 0$. While reducing $\oursigma$ improves throughput, it considerably increases the communication \textit{burstiness}, as described in Section~\ref{sec:distributed}.
In general, increased burstiness means that the long term throughput can be achieved with given power budgets but the variance is more significant during short term intervals. Recall from Section~\ref{ssec:sim-setup} that the packet length is $\ourms{1}$, we therefore measure the average burst length compared to this unit packet length.

%%
% path: ./fig/sim_figs/
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.8\columnwidth]{figs/sim_figs/sim_burstiness.pdf}
\caption{Average burst length obtained analytically (curves) and via simulation (markers) with $\numnode \in \{5, 10\}$, $\oursigma \in \{0.25, 0.5\}$, $\energybound{} = \ouruW{10}$, and $\listencost{} = \xmitcost{} = \ouruW{500}$.}
\label{fig:sim-avg-pkt-len}
\vspace{-1.5\baselineskip}
\end{center}
\end{figure}

Figure~\ref{fig:sim-avg-pkt-len} shows the average burst length received by the nodes in homogeneous networks with $\numnode \in \{5, 10\}$, $\energybound{} = \ouruW{10}$, $\listencost{} = \xmitcost{} = \ouruW{500}$, and varying $\oursigma$. Values are extracted using an analytical formula (curves) derived from the solution of {\namecp} and contrasted with simulations at specific values of $\oursigma$ (markers). Aside from showing that the simulation results and the analytical results are well matched, Figure~\ref{fig:sim-avg-pkt-len} also demonstrates how reducing $\oursigma$ dramatically increases burstiness. For example, with $\oursigma = 0.25$ and $\numnode = 10$, a node has an average received burst length of $\ourms{85}$, and this value is increased to $\ourms{4.5e5}$ with $\oursigma = 0.1$. This explains why $\gputsigmasim$ cannot be obtained with $\oursigma = 0.1$ (see Section~\ref{ssec:sim-setup}) and we remark that reducing the communication burstiness is a subject of future work.

%%
% path: ./fig/sim_figs/
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.8\columnwidth]{figs/sim_figs/sim_latency_cdf.eps}
\caption{The CDF, mean, and $99^{\rm th}$ percentile latency of {\name} obtained via simulation with $\numnode \in \{5, 10\}$, $\oursigma \in \{0.25, 0.5\}$, $\energybound{} = \ouruW{10}$, and $\listencost{} = \xmitcost{} = \ouruW{500}$, compared to the pairwise worst case latency of Searchlight.}
\label{fig:sim-latency-cdf}
\vspace{-1.5\baselineskip}
\end{center}
\end{figure}

A second metric we consider is the communication \textit{latency}. It is defined as the time interval between consecutive bursts received by a node from some other node where the interval includes \textit{at least} one sleep period. We focus on this metric because nodes receiving longer bursts consume more energy, and therefore, need to sleep for longer periods of time. It is possible for a node to receive multiple bursts in one listen period.
%\comments{TC: is this clear about why are do we need a sleep during the latency?}
Figure~\ref{fig:sim-latency-cdf} presents the CDF of communication latency obtained via simulations, for $\numnode \in \{5, 10\}$ and $\oursigma \in \{0.25, 0.5\}$, and indicates both the average and the $99^{\rm th}$-percentile latency values. It also shows the pairwise worst case latency of Searchlight computed from~\cite{Bakht_mobicom2012} under the same power consumption level and power budget.\footnote{This is computed with slot length of $\ourms{50}$ and a beacon (packet) length of $\ourms{1}$ as was done in~\cite{sun2014hello}.}

Figure~\ref{fig:sim-latency-cdf} shows that (i) as $\oursigma$ decreases, the latency increases since nodes suffering from long bursts will sleep longer, and (ii) larger value of $\numnode$ results in lower latency, since it is more likely to receive when more nodes exist. As an example, with $\oursigma = 0.5$ and $\numnode = 5$, a node receives bursts from some other node on average every $5$ seconds. In addition, for all parameters considered, the $99^{\rm th}$-percentile latency is within $120$ seconds, outperforming the Searchlight pairwise worst case latency bound of $125$ seconds. Note that although {\name} has a non-zero probability of having any latency, in most cases (over $99\%$), its latency is below the worst case latency of Searchlight.


%%
% - non-clique setup
% - non-clique tput and upper bounds
\subsection{Evaluation in Non-clique Topologies}
\label{ssec:sim-nonclique}

%%
% path: ./fig/analysis_figs/
\begin{figure}[!t]
\begin{center}
\includegraphics[width=0.8\columnwidth]{figs/sim_figs/sim_tput_non_clique_grid.pdf}
\caption{The oracle throughput in non-clique topologies, $\UBNC$, and the throughput of {\name} obtained via simulations, $\gputsigmasim$, in grid topologies with varying $\numnode$ and $\oursigma$.}
\label{fig:sim-tput-non-clique-grid}
\vspace{-1.5\baselineskip}
\end{center}
\end{figure}

We now compute the oracle throughput for non-clique topologies (derived in Section~\ref{ssec:upper-additional}) and evaluate the throughput of {\name} in such scenarios. Operating in a distributed manner, {\name} can be easily adapted to non-clique topologies: if a node hears two simultaneous transmissions from two nodes, it does not count any of the transmissions as throughput. Recall from Section~\ref{sec:formulation} that nodes always check the channel utilization before waking up, simultaneous transmission can only happen if two nodes are not within communication range of each other.

We use grid topologies with varying number of nodes, $\numnode$, in which a node can only have at most $4$ neighbors. For example, $\numnode=25$ represents a $5 \times 5$ grid. For each value of $N$, we compute the oracle throughput (groupput). Figure~\ref{fig:sim-tput-non-clique-grid} presents the oracle throughput, $\UBNC$, for grid topologies, and the throughput achieved by {\name} via simulations with with varying $\oursigma$. Note that for all the grid topologies considered, the upper and lower bounds of $\UBNC$ (see Section~\ref{ssec:upper-additional}) are the same, providing the exact oracle throughput.


Figure~\ref{fig:sim-tput-non-clique-grid} shows that {\name} achieves $14\% - 22\%$ of the maximum throughput $\UBNC$ with $\oursigma = 0.25$. Although increasing $\oursigma$ leads to lower throughput, it can be observed that as $\numnode$ increases, the throughput approaches $10\%$ of $\UBNC$ with $\oursigma = 0.5$. Although we cannot obtain the throughput for $\oursigma = 0.1$, achieving $10\% - 20\%$ of $\UBNC$ is remarkable given the fact that {\name} works in a distributed manner in which each node does not have any information of the properties of other nodes.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../conext16"
%%% End: 
